Asymmetric Trust Effects of Corrective AI in Expert Advisory Workflows under Epistemic Dependence

The increasing integration of AI-powered tools into expert workflows, such as medicine, law, and finance, raises a critical question: how does AI involvement influence a user`s trust in the human expert, the AI system, and the human-AI team? This question is especially important in expert advisory settings where users are epistemically dependent on human-AI systems: they are recipients of guidance produced by an expert using AI support, but often lack the domain knowledge needed to independently verify the recommendation. We investigated these dynamics through a user study (N=157) using a simulated course-planning task. Our design varied advisor performance and the structure of AI involvement, including whether AI support was present and, when present, whether it was invoked by the advisor or automatically monitored the interaction. Across all conditions, workflows ultimately produced correct schedules. Results show an asymmetric trust effect: advisor errors significantly reduce trust in the human advisor, but visible AI correction does not produce a corresponding increase in trust toward the AI assistant. Trust judgments remain anchored to the advisor across multiple trust measures, and changing the visible structure of AI involvement does not substantially redistribute trust toward the AI assistant or the human-AI team. These findings suggest a limit of corrective AI as a governance mechanism: making AI oversight visible may improve workflow recoverability, but it does not necessarily redistribute trust or responsibility away from the human-facing expert. In epistemically dependent settings, correctness alone may be insufficient for trustworthy AI integration, as users may continue to assign responsibility to the human expert even when AI assistance visibly shapes the final outcome.

==> Dennis-sections/Results/analysis.tex <==
\subsection{Overview of Analytical Approach}

\textcolor{blue}{For advisor-directed measures, we conducted 3 × 2 factorial ANOVAs testing advisor performance (error vs. errorless), AI intervention modality (none, proactive, reactive), and their interaction. Because AI-assistant and advisor-AI-team ratings were collected only in the AI-supported conditions, those outcomes were analyzed using 2 × 2 factorial ANOVAs testing advisor performance, AI intervention modality (proactive vs. reactive), and their interaction.} These analyses evaluated the hypotheses: advisor performance effects tested H1 and H4, AI modality main effects tested H2, and advisor performance by modality interactions tested H3. Outcomes included epistemic trustworthiness composites (expertise, integrity, benevolence~\cite{hendriks2015meti}), entity-level trust adapted from~\citet{riedl2024patients}, a 1 to 100 general trust rating, and likelihood of advisor reuse. Tukey’s HSD pairwise comparisons were conducted as exploratory analyses across all condition combinations. Effect sizes are reported as $\eta^2$ and Cohen’s $d$, with test statistics in standard ANOVA form and exact degrees of freedom. Variance differences between error-present and errorless conditions were assessed using Levene’s test.

\subsection{Omnibus Tests Across Trust Constructs}
\label{subsec:omnibus}

We first report the full 3$\times$2 factorial analyses, which provide the primary basis for evaluating the hypotheses.

\textbf{Advisor-directed trust~\cite{riedl2024patients}.} Performance significantly reduced evaluations in error conditions across perceived trustworthiness (``The advisor is trustworthy''), information trustworthiness (``I can trust the information presented by the advisor''), and affective comfort (``I have a good feeling when relying on the advisor''): perceived trustworthiness, $F(1,151)=13.0$, $p<.001$, $\eta^2=0.08$; affective comfort, $F(1,151)=22.5$, $p<.001$, $\eta^2=0.13$; information trustworthiness, $F(1,151)=19.6$, $p<.001$, $\eta^2=0.11$. These results support H1. General trust showed the same pattern, $F(1,151)=21.14$, $p<.001$, $\eta^2=0.12$, further supporting H1. Likelihood of advisor reuse was also lower in error-present conditions, $F(1,151)=26.29$, $p<.001$, $\eta^2=0.15$, supporting H4.

\textbf{Epistemic trustworthiness~\cite{hendriks2015meti}.} Performance significantly affected perceived expertise, integrity, and benevolence of the advisor, with higher evaluations in errorless conditions than in error-present conditions. Since H1 concerns the effect of advisor errors relative to errorless performance, these METI comparisons directly support H1: expertise, $F(1,151)=21.89$, $p<.001$, $\eta^2=0.13$; integrity, $F(1,151)=8.80$, $p=.004$, $\eta^2=0.06$; benevolence, $F(1,151)=6.92$, $p=.009$, $\eta^2=0.04$. These METI results further support H1.

\textbf{AI-supported conditions (2$\times$2 analysis)~\cite{riedl2024patients}.} Restricting analyses to AI-supported conditions showed the same performance-driven pattern for the advisor across all Riedl items: perceived trustworthiness, $F(1,105)=9.34$, $p=.003$, $\eta^2=0.08$; affective comfort, $F(1,105)=12.7$, $p<.001$, $\eta^2=0.11$; information trustworthiness, $F(1,105)=12.8$, $p<.001$, $\eta^2=0.11$. These results show that support for H1 persisted within AI-supported workflows.

This pattern was less consistent for the advisor-AI combination: team trustworthiness, $F(1,105)=4.16$, $p=.044$, $\eta^2=0.04$; information trustworthiness, $F(1,105)=7.07$, $p=.009$, $\eta^2=0.06$; affective comfort, $F(1,105)=3.75$, $p=.056$, $\eta^2=0.03$. No significant effects were observed for trust in the AI assistant alone (all $p>.05$).

No significant main effects of AI intervention modality were observed over any of these instruments; thus, H2 was not supported. Specifically, AI modality did not significantly redistribute trust-related evaluations across the advisor, AI assistant, and advisor-AI team, nor increase evaluations of the AI assistant or advisor-AI team. No significant advisor performance by modality interactions were observed, so H3 was not supported.

\subsection{Descriptive Statistics}

Descriptive statistics for all trust constructs are reported in Appendix~\ref{app:descriptive_tables}. Error-present conditions were evaluated less favorably than errorless conditions across advisor measures, consistent with H1 and H4; AI modality differences were small and showed no consistent directional pattern, consistent with the lack of support for H2 and H3. Error-present conditions also exhibited greater variability for several measures (e.g., expertise). Significant Levene’s test results were observed only for advisor-directed measures, with no significant variance differences for the AI assistant or combined team (Appendix~\ref{app:variance_tables}). These exploratory variance analyses were not primary tests of the hypotheses.

\subsection{Pairwise Condition Comparisons}

Tukey HSD pairwise comparisons were exploratory, as factorial ANOVAs provide the primary basis for inference. Mean differences are computed as (condition$_2$ $-$ condition$_1$), such that negative values indicate higher ratings in the first-listed condition.

\textbf{Epistemic expertise~\cite{hendriks2015meti}.} Ratings were lower in \advonlyerr{} relative to \advonly{} ($d=.914$, $p=.025$) and in \procfail{} relative to \procsucc{} ($d=.798$, $p=.023$). Additionally, \advonly{} achieved higher evaluations than \procfail{} ($d=-1.05$, $p=.004$).

\textbf{Advisor-directed trust~\cite{riedl2024patients}.} For affective comfort, \advonlyerr{} was lower than \advonly{} ($d=0.91$, $p=.005$), \reactsucc{} ($d=1.13$, $p<.001$), and \procsucc{} ($d=1.04$, $p=.001$); \reactsucc{} was also rated higher than \procfail{} ($d=-0.81$, $p=.046$). For information trustworthiness, \advonlyerr{} was lower than \reactsucc{} ($d=0.84$, $p=.039$), and \procfail{} was lower than \advonly{} ($d=0.79$, $p=.041$) and \reactsucc{} ($d=0.87$, $p=.021$).

\textbf{AI-supported conditions (2$\times$2 analysis)~\cite{riedl2024patients}.} For affective comfort, \reactsucc{} was rated higher than \procfail{} ($d=-0.81$, $p=.011$), and \procfail{} was lower than \procsucc{} ($d=0.73$, $p=.017$). For information trustworthiness, \reactsucc{} exceeded \procfail{} ($d=-.87$, $p=.007$), and \procfail{} was lower than \procsucc{} ($d=.65$, $p=.046$).

\textbf{General trust and advisor reuse.} Reuse was lower in \advonlyerr{} relative to \advonly{} ($d=1.25$, $p<.001$), \reactsucc{} ($d=0.97$, $p=.004$), and \procsucc{} ($d=1.11$, $p<.001$), and lower in \procfail{} relative to \procsucc{} ($d=0.80$, $p=.036$), while higher in \advonly{} compared to \procfail{} ($d=-0.95$, $p=.011$). General trust was lower in \advonlyerr{} relative to \advonly{} ($d=1.03$, $p=.010$), \reactsucc{} ($d=0.89$, $p=.021$), and \procsucc{} ($d=0.94$, $p=.009$), as well as in \procfail{} relative to \procsucc{} ($d=0.74$, $p=.047$), and higher in \advonly{} compared to \procfail{} ($d=-0.82$, $p=.047$).

Overall, exploratory pairwise comparisons were consistent with the omnibus tests: significant differences primarily reflected error-present versus errorless contrasts, supporting H1 and H4, rather than reliable AI modality differences or advisor performance by modality interactions, which would have supported H2 or H3.

==> Dennis-sections/Results/summary.tex <==
\subsection{Summary of Results}

Across analyses, advisor errors significantly reduced advisor-directed trust evaluations, including epistemic trustworthiness~\cite{hendriks2015meti}, entity-specific trust~\cite{riedl2024patients}, general trust, and likelihood of advisor reuse. These results support H1 and H4.

No significant AI modality main effects were observed, so H2 was not supported: AI intervention modality did not significantly redistribute trust-related consequences across advisor-directed, AI-directed, and team-directed measures or shift evaluations toward the AI assistant or advisor-AI team. No significant differences in advisor performance evaluations were observed across modality interactions, so H3 was not supported. \textcolor{blue}{The 3 × 2 interaction analyses had approximately 79.9\% power to detect a medium interaction effect (f=.25). The restricted 2 × 2 interaction analyses had approximately 73.4\% power under the same effect-size assumption; therefore, particularly for the AI-supported outcomes, the nonsignificant interaction results do not rule out smaller interaction effects.} Pairwise comparisons were consistent with this pattern and primarily reflected error-present versus errorless contrasts.

==> Dennis-sections/appendices.tex <==
\clearpage

\appendix

\section{Results Details}
\subsection{Survey Measures and Reliability}
\label{app:measures}
Summary of survey measures and reliability is provided in Table~\ref{tab:measures_items}.

\begin{table}[!htbp]
\centering
\setlength{\tabcolsep}{1mm}
\begin{tabular}{lcc}
\toprule
\textbf{Construct} & \textbf{Items} & \textbf{Cronbach's $\boldsymbol{\alpha}$} \\
\midrule
METI Expertise & 7 & 0.91 \\
METI Integrity & 5 & 0.82 \\
METI Benevolence & 4 & 0.90 \\
Advisor Trust (Riedl) & 3 & $>0.70$ \\
AI Trust (Riedl) & 3 & $>0.70$ \\
Advisor/AI Trust (Riedl) & 3 & $>0.70$ \\
\bottomrule
\end{tabular}
\caption{Reliability of trust-related composites}
\label{tab:measures_items}
\end{table}
%\FloatBarrier

\subsection{METI Items and Dimensional Structure}
\label{app:meti}
\begin{figure}[ht]
  \centering
  \includegraphics[width=\linewidth]{meti_items.png}
  \caption{Items and dimensional structure of the Muenster Epistemic Trustworthiness Inventory (METI), sourced from \citet{hendriks2015meti}}
  \label{fig:meti_items}
\end{figure}
%\FloatBarrier



\subsection{Participant breakdowns by condition}
\label{app:participant-breakdowns}
We report participant demographic breakdowns by condition in Tables~\ref{tab:ai_use_freq_by_condition}, \ref{tab:age_by_condition}, \ref{tab:educ_by_condition}, and \ref{tab:gender_by_condition}.

\begin{table*}[htbp]
\centering
\setlength{\tabcolsep}{1mm}
\begin{tabular}{l r c c c c}
\toprule
\textbf{Condition} & \textbf{N} & \textbf{Annually} & \textbf{Daily} & \textbf{Monthly} & \textbf{Weekly} \\
\midrule
\advonly    & 22 & 2 (9.1\%) & 8 (36.4\%)  & 1 (4.5\%)  & 11 (50.0\%) \\
\advonlyerr & 26 & 2 (7.7\%) & 11 (42.3\%) & 3 (11.5\%) & 10 (38.5\%) \\
\reactfail  & 25 & 0 (0.0\%) & 14 (56.0\%) & 3 (12.0\%) & 8 (32.0\%) \\
\reactsucc  & 27 & 2 (7.4\%) & 12 (44.4\%) & 3 (11.1\%) & 10 (37.0\%) \\
\procfail   & 28 & 1 (3.6\%) & 11 (39.3\%) & 6 (21.4\%) & 10 (35.7\%) \\
\procsucc   & 29 & 0 (0.0\%) & 9 (31.0\%)  & 2 (6.9\%)  & 18 (62.1\%) \\
\bottomrule
\end{tabular}
\caption{AI use frequency by condition (n, row \%).}
\label{tab:ai_use_freq_by_condition}
\end{table*}

\begin{table*}[htbp]
\centering
\setlength{\tabcolsep}{1mm}
\begin{tabular}{l r c c c c c c}
\toprule
\textbf{Condition} & \textbf{N} & \textbf{18--24} & \textbf{25--34} & \textbf{35--44} & \textbf{45--54} & \textbf{55--64} & \textbf{65+} \\
\midrule
\advonly    & 22 & 1 (4.5\%)  & 11 (50.0\%) & 3 (13.6\%)  & 4 (18.2\%)  & 2 (9.1\%)  & 1 (4.5\%) \\
\advonlyerr & 26 & 2 (7.7\%)  & 4 (15.4\%)  & 13 (50.0\%) & 4 (15.4\%)  & 2 (7.7\%)  & 1 (3.8\%) \\
\reactfail  & 25 & 1 (4.0\%)  & 9 (36.0\%)  & 9 (36.0\%)  & 1 (4.0\%)   & 5 (20.0\%) & 0 (0.0\%) \\
\reactsucc  & 27 & 6 (22.2\%) & 9 (33.3\%)  & 8 (29.6\%)  & 3 (11.1\%)  & 1 (3.7\%)  & 0 (0.0\%) \\
\procfail   & 28 & 3 (10.7\%) & 11 (39.3\%) & 9 (32.1\%)  & 3 (10.7\%)  & 2 (7.1\%)  & 0 (0.0\%) \\
\procsucc   & 29 & 4 (13.8\%) & 12 (41.4\%) & 3 (10.3\%)  & 3 (10.3\%)  & 4 (13.8\%) & 3 (10.3\%) \\
\bottomrule
\end{tabular}
\caption{Age by condition (n, row \%).}
\label{tab:age_by_condition}
\end{table*}


\begin{table*}[htbp]
\centering
\setlength{\tabcolsep}{1mm}

\begin{tabular}{l r c c c c c c}
\toprule
\textbf{Condition} & \textbf{N} & \textbf{Associate} & \textbf{Some college} & \textbf{Bachelor's} & \textbf{Doctorate} & \textbf{High school (or equiv.)} & \textbf{Master's} \\
\midrule
\advonly    & 22 & 0 (0.0\%)  & 3 (13.6\%) & 9 (40.9\%)  & 1 (4.5\%) & 4 (18.2\%)  & 5 (22.7\%) \\
\advonlyerr & 26 & 3 (11.5\%) & 6 (23.1\%) & 8 (30.8\%)  & 1 (3.8\%) & 2 (7.7\%)   & 6 (23.1\%) \\
\reactfail  & 25 & 2 (8.0\%)  & 4 (16.0\%) & 10 (40.0\%) & 1 (4.0\%) & 4 (16.0\%)  & 4 (16.0\%) \\
\reactsucc  & 27 & 4 (14.8\%) & 6 (22.2\%) & 11 (40.7\%) & 1 (3.7\%) & 3 (11.1\%)  & 2 (7.4\%) \\
\procfail   & 28 & 3 (10.7\%) & 4 (14.3\%) & 11 (39.3\%) & 2 (7.1\%) & 1 (3.6\%)   & 7 (25.0\%) \\
\procsucc   & 29 & 4 (13.8\%) & 8 (27.6\%) & 7 (24.1\%)  & 2 (6.9\%) & 6 (20.7\%)  & 2 (6.9\%) \\
\bottomrule
\end{tabular}
\caption{Education by condition (n, row \%).}
\label{tab:educ_by_condition}
\end{table*}

\begin{table*}[htbp]
\centering
\setlength{\tabcolsep}{1mm}
\begin{tabular}{l r c c c}
\toprule
\textbf{Condition} & \textbf{N} & \textbf{Man} & \textbf{Woman} & \textbf{Prefer not to say} \\
\midrule
\advonly    & 22 & 11 (50.0\%) & 10 (45.5\%) & 1 (4.5\%) \\
\advonlyerr & 26 & 14 (53.8\%) & 12 (46.2\%) & 0 (0.0\%) \\
\reactfail  & 25 & 15 (60.0\%) & 10 (40.0\%) & 0 (0.0\%) \\
\reactsucc  & 27 & 13 (48.1\%) & 14 (51.9\%) & 0 (0.0\%) \\
\procfail   & 28 & 19 (67.9\%) & 9 (32.1\%)  & 0 (0.0\%) \\
\procsucc   & 29 & 18 (62.1\%) & 11 (37.9\%) & 0 (0.0\%) \\
\bottomrule
\end{tabular}
\caption{Gender by condition (n, row \%).}
\label{tab:gender_by_condition}
\end{table*}


\subsection{Descriptive Statistics}
\label{app:descriptive_tables}
% {Note that for METI dimensions, the reported means are combined over that dimension's items.}
Note that for METI dimensions, the reported means are averaged across items within each dimension. Results are shown in Tables~\ref{tab:meti_means}, \ref{tab:reuse_means}, and \ref{tab:riedl_3x2}.

\begin{table}[htbp]
\centering
\setlength{\tabcolsep}{1mm}
\begin{tabular}{llcc}
\toprule
\textbf{Response Variable} & \textbf{Modality} & \textbf{Fail} & \textbf{No Error} \\
\midrule
Expertise   & No-AI & 5.37 (1.32) & 6.38 (0.76) \\
Expertise   & Reactive          & 5.45 (1.28) & 6.01 (0.79) \\
Expertise   & Proactive          & 5.20 (1.34) & 6.13 (0.98) \\
\midrule
Integrity   & No-AI & 5.52 (1.02) & 6.08 (0.97) \\
Integrity   & Reactive          & 5.78 (0.87) & 6.00 (0.88) \\
Integrity   & Proactive          & 5.73 (0.93) & 6.23 (0.75) \\
\midrule
Benevolence & No-AI & 5.37 (1.20) & 5.77 (1.02) \\
Benevolence & Reactive          & 5.36 (1.25) & 5.77 (1.01) \\
Benevolence & Proactive          & 5.37 (1.10) & 5.94 (1.08) \\
\bottomrule
\end{tabular}
\caption{Means (standard deviations) for METI dimensions by AI modality and advisor performance}
\label{tab:meti_means}
\end{table}

\begin{table*}[htbp]
\centering
\setlength{\tabcolsep}{1mm}
\begin{tabular}{llcc}
\toprule
\textbf{Response Variable} & \textbf{Modality} & \textbf{Fail} & \textbf{No Error} \\
\midrule
Reuse         & No-AI & 4.39 (1.86) & 6.36 (1.18) \\
Reuse         & Reactive          & 5.32 (1.63) & 5.93 (1.27) \\
Reuse         & Proactive          & 4.89 (1.79) & 6.10 (1.21) \\
\midrule
General Trust & No-AI & 63.92 (23.31) & 84.55 (15.27) \\
General Trust & Reactive          & 72.56 (23.72) & 82.19 (17.52) \\
General Trust & Proactive          & 67.25 (24.86) & 83.31 (17.87) \\
\bottomrule
\end{tabular}
\caption{Means (standard deviations) for reuse and general trust by AI modality and advisor performance}
\label{tab:reuse_means}
\end{table*}

\begin{table*}[htbp]
\centering
\setlength{\tabcolsep}{1mm}
\begin{tabular}{llcc}
\toprule
\textbf{Response Variable} & \textbf{Modality} & \textbf{Fail} & \textbf{No Error} \\
\midrule
Advisor is trustworthy        & No-AI & 5.27 (1.56) & 6.09 (1.34) \\
Advisor is trustworthy        & Reactive          & 5.44 (1.56) & 6.11 (0.93) \\
Advisor is trustworthy        & Proactive          & 5.29 (1.58) & 6.10 (0.90) \\
\midrule
Trust advisor's information   & No-AI & 5.27 (1.56) & 6.27 (0.99) \\
Trust advisor's information   & Reactive          & 5.48 (1.36) & 6.30 (0.78) \\
Trust advisor's information   & Proactive          & 5.21 (1.57) & 6.07 (1.03) \\
\midrule
Comfort relying on advisor    & No-AI & 4.46 (1.94) & 6.00 (1.35) \\
Comfort relying on advisor    & Reactive          & 5.40 (1.47) & 6.15 (0.86) \\
Comfort relying on advisor    & Proactive          & 5.00 (1.79) & 6.07 (1.07) \\
\bottomrule
\end{tabular}
\caption{Means (standard deviations) for advisor-directed trust (Riedl items) across all conditions}
\label{tab:riedl_3x2}
\end{table*}

\subsection{Omnibus Test Statistics}
\label{app:omnibus-tests}

The factorial ANOVAs reported in the main text provide the primary basis for inference. This section reports the complete omnibus statistics for advisor-directed, epistemic trustworthiness, and AI-supported analyses.

\textbf{Full 3$\times$2 analysis: advisor-directed trust~\cite{riedl2024patients}.}

Advisor performance significantly affected perceived trustworthiness, $F(1,151)=13.0$, $p<.001$, $\eta^2=0.08$; affective comfort, $F(1,151)=22.5$, $p<.001$, $\eta^2=0.13$; and information trustworthiness, $F(1,151)=19.6$, $p<.001$, $\eta^2=0.11$. General trust showed the same pattern, $F(1,151)=21.14$, $p<.001$, $\eta^2=0.12$. Likelihood of advisor reuse was also lower in error-present conditions, $F(1,151)=26.29$, $p<.001$, $\eta^2=0.15$.

\textbf{Full 3$\times$2 analysis: epistemic trustworthiness~\cite{hendriks2015meti}.}

Advisor performance significantly affected expertise, $F(1,151)=21.89$, $p<.001$, $\eta^2=0.13$; integrity, $F(1,151)=8.80$, $p=.004$, $\eta^2=0.06$; and benevolence, $F(1,151)=6.92$, $p=.009$, $\eta^2=0.04$.

\textbf{AI-supported conditions (2$\times$2 analysis)~\cite{riedl2024patients}.}

Restricting analyses to AI-supported conditions, advisor performance significantly affected advisor perceived trustworthiness, $F(1,105)=9.34$, $p=.003$, $\eta^2=0.08$; affective comfort, $F(1,105)=12.7$, $p<.001$, $\eta^2=0.11$; and information trustworthiness, $F(1,105)=12.8$, $p<.001$, $\eta^2=0.11$.

Advisor-AI team evaluations showed significant effects for perceived trustworthiness, $F(1,105)=4.16$, $p=.044$, $\eta^2=0.04$, and information trustworthiness, $F(1,105)=7.07$, $p=.009$, $\eta^2=0.06$, but not affective comfort, $F(1,105)=3.75$, $p=.056$, $\eta^2=0.03$.

No significant advisor performance effects were observed for AI assistant trust measures (all $p>.05$).

No significant main effects of AI intervention modality were observed across measures. No significant advisor performance by modality interactions were observed.

\subsection{Bayesian ANOVA Results}
\label{app:bayesian-anovas}

To provide additional evidence regarding the unsupported H2 and H3 hypotheses, we conducted Bayesian ANOVAs on AI-supported trust evaluations using JASP's default JZS Bayes factor approach with Cauchy priors. Values of $BF_{\mathrm{excl}}$ quantify evidence favoring exclusion of the corresponding effect from the model, with larger values indicating stronger evidence against including the effect (refer to table \ref{tab:bayesian-anovas}).


\begin{table*}[htbp]
\centering
\setlength{\tabcolsep}{1mm}
\begin{tabular}{p{7.2cm}cc}
\toprule
\textbf{Dependent Variable} & 
$BF_{\mathrm{excl}}$ (AI Modality) &
$BF_{\mathrm{excl}}$ (AI Modality $\times$ Performance) \\
\midrule
The AI assistant is trustworthy 
& 6.376 & 13.460 \\
I have a good feeling when relying on the AI assistant 
& 4.841 & 5.712 \\
I can trust the information presented by the AI assistant 
& 6.742 & 14.530 \\
The advisor and AI assistant combination is trustworthy 
& 5.705 & 6.818 \\
I have a good feeling when relying on the advisor and AI assistant combination 
& 6.305 & 8.884 \\
I can trust the information presented by the advisor and AI assistant combination 
& 6.081 & 5.612 \\
The advisor is trustworthy 
& 5.729 & 5.307 \\
I have a good feeling when relying on the advisor 
& 3.847 & 3.618 \\
I can trust the information presented by the advisor 
& 3.662 & 3.718 \\
\bottomrule
\end{tabular}
\caption{Bayesian ANOVA results for AI-supported trust evaluations.}
\label{tab:bayesian-anovas}
\end{table*}

\subsection{Exploratory Pairwise Condition Comparisons}
\label{app:pairwise-comparisons}

Table~\ref{tab:pairwise-comparisons} reports the significant exploratory
Tukey HSD comparisons. Factorial ANOVAs provide the primary basis for
inference. Mean differences were computed as condition$_2-$condition$_1$.
Thus, negative values indicate higher ratings in the first-listed condition.

\begin{table*}[htbp]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{p{4.4cm}llcc}
\toprule
\textbf{Outcome / Analysis}
& \textbf{Condition$_1$}
& \textbf{Condition$_2$}
& $\boldsymbol{d}$
& $\boldsymbol{p}$ \\
\midrule

Epistemic expertise
& \advonlyerr{} & \advonly{} & .914 & .025 \\
& \procfail{} & \procsucc{} & .798 & .023 \\
& \advonly{} & \procfail{} & $-1.05$ & .004 \\

\midrule
Affective comfort (full 3$\times$2)
& \advonlyerr{} & \advonly{} & .91 & .005 \\
& \advonlyerr{} & \reactsucc{} & 1.13 & $<.001$ \\
& \advonlyerr{} & \procsucc{} & 1.04 & .001 \\
& \reactsucc{} & \procfail{} & $-.81$ & .046 \\

\midrule
Information trustworthiness (full 3$\times$2)
& \advonlyerr{} & \reactsucc{} & .84 & .039 \\
& \procfail{} & \advonly{} & .79 & .041 \\
& \procfail{} & \reactsucc{} & .87 & .021 \\

\midrule
Affective comfort (AI-supported 2$\times$2)
& \reactsucc{} & \procfail{} & $-.81$ & .011 \\
& \procfail{} & \procsucc{} & .73 & .017 \\

\midrule
Information trustworthiness (AI-supported 2$\times$2)
& \reactsucc{} & \procfail{} & $-.87$ & .007 \\
& \procfail{} & \procsucc{} & .65 & .046 \\

\midrule
Advisor reuse
& \advonlyerr{} & \advonly{} & 1.25 & $<.001$ \\
& \advonlyerr{} & \reactsucc{} & .97 & .004 \\
& \advonlyerr{} & \procsucc{} & 1.11 & $<.001$ \\
& \procfail{} & \procsucc{} & .80 & .036 \\
& \advonly{} & \procfail{} & $-.95$ & .011 \\

\midrule
General trust
& \advonlyerr{} & \advonly{} & 1.03 & .010 \\
& \advonlyerr{} & \reactsucc{} & .89 & .021 \\
& \advonlyerr{} & \procsucc{} & .94 & .009 \\
& \procfail{} & \procsucc{} & .74 & .047 \\
& \advonly{} & \procfail{} & $-.82$ & .047 \\

\bottomrule
\end{tabular}
\caption{Significant exploratory Tukey HSD pairwise comparisons. Differences
were computed as condition$_2-$condition$_1$; negative values therefore
indicate higher ratings in condition$_1$. Only statistically significant
comparisons are shown.}
\label{tab:pairwise-comparisons}
\end{table*}




\subsection{Variance Differences Across Performance Conditions}
\label{app:variance_tables}

To examine whether advisor errors were associated not only with lower trust
but also with greater heterogeneity in responses, we compared response
variability between error-present and errorless conditions using Levene’s test. 

\paragraph{Primary analysis (full sample).}
Table~\ref{tab:levene_main} reports Levene’s test results for the primary
full-sample analysis of aggregate trust-related measures.

\begin{table*}[ht]
\centering
\setlength{\tabcolsep}{1mm}
\begin{tabular}{lcccc}
\toprule
\textbf{Response Variable} & \textbf{Error-present SD} & \textbf{Errorless SD} & $\boldsymbol{W}$ & $\boldsymbol{p}$ \\
\midrule
Expertise      & 1.303 & 0.862 & 17.46 & $< .001$ \\
Integrity      & 0.938 & 0.856 & 1.83  & .179 \\
Benevolence    & 1.168 & 1.028 & 1.49  & .224 \\
Reuse          & 1.781 & 1.217 & 10.15 & .002 \\
General Trust  & 23.949 & 16.859 & 11.19 & .001 \\
\bottomrule
\end{tabular}
\caption{Levene’s tests comparing response variability between error-present and errorless conditions in the primary full-sample analysis ($n = 79$ error-present, $n = 78$ errorless).}
\label{tab:levene_main}
\end{table*}

\paragraph{Reduced 2$\times$2 item-level analysis.}
Table~\ref{tab:levene_2x2} reports Levene’s test results for entity-level
trust measures in AI-supported conditions, where the advisor, AI assistant, and
advisor-AI team were all present.

\begin{table*}[tbp]
\centering
\setlength{\tabcolsep}{1mm}
\begin{tabular}{lcccc}
\toprule
\textbf{Response Variable} & \textbf{Error-present SD} & \textbf{Errorless SD} & $\boldsymbol{W}$ & $\boldsymbol{p}$ \\
\midrule
AI Assistant Perceived Trustworthiness & 1.348 & 1.206 & 0.07 & .799 \\
AI Assistant Affective Comfort & 1.669 & 1.628 & 0.62 & .433 \\
AI Assistant Information Trustworthiness & 1.307 & 1.345 & 0.04 & .837 \\
Advisor-AI Perceived Trustworthiness & 1.552 & 1.197 & 1.16 & .283 \\
Advisor-AI Affective Comfort & 1.680 & 1.381 & 2.53 & .114 \\
Advisor-AI Information Trustworthiness & 1.419 & 1.135 & 2.36 & .127 \\
Advisor Perceived Trustworthiness & 1.558 & 0.908 & 6.77 & .011 \\
Advisor Affective Comfort & 1.641 & 0.966 & 5.31 & .023 \\
Advisor Information Trustworthiness & 1.467 & 0.917 & 8.39 & .005 \\
\bottomrule
\end{tabular}
\caption{Levene’s tests comparing response variability between error-present and errorless conditions for entity-level trust measures in the reduced 2$\times$2 AI-supported analysis ($n = 53$ error-present, $n = 56$ errorless).}
\label{tab:levene_2x2}
\end{table*}

\paragraph{Full 3$\times$2 item-level analysis.}
Table~\ref{tab:levene_3x2} reports Levene’s test results for advisor-directed measures across the full 3$\times$2 design.

\begin{table*}[tbp]
\centering
\setlength{\tabcolsep}{1mm}
\begin{tabular}{lcccc}
\toprule
\textbf{Response Variable} & \textbf{Error-present SD} & \textbf{Errorless SD} & $\boldsymbol{W}$ & $\boldsymbol{p}$ \\
\midrule
Advisor Perceived Trustworthiness & 1.550 & 1.039 & 9.36  & .003 \\
Advisor Affective Comfort & 1.768 & 1.078 & 18.74 & $< .001$ \\
Advisor Information Trustworthiness & 1.490 & 0.931 & 14.22 & $< .001$ \\
\bottomrule
\end{tabular}
\caption{Levene’s tests comparing response variability between error-present and errorless conditions for advisor-directed item-level measures in the full 3$\times$2 analysis ($n = 79$ error-present, $n = 78$ errorless).}
\label{tab:levene_3x2}
\end{table*}

\noindent\textit{Note.} Across analyses, error-present conditions exhibited
greater variability than errorless conditions with regard to the advisor-trust measures.



\section{Questionnaire Details}
\subsection{\citet{hendriks2015meti} METI trustworthiness items}
\label{app:meti-items}

Participants completed this Muenster Epistemic Trustworthiness Inventory (METI) \citep{hendriks2015meti}. Items were grouped into three dimensions: expertise, integrity, and benevolence.
\begin{itemize}
  \item Expertise items:
    \begin{itemize}
      \item How competent did you feel your advisor was in constructing the most suitable course schedule for you? 
      \item How would you rate the advisor’s intelligence based on the interaction and course scheduling process?
      \item Based on your interaction, how educated did the advisor seem?
      \item How professional was your interaction with your advisor while constructing your curriculum?
      \item Based on the process, how experienced did the advisor seem while structuring your schedule?
      \item How qualified was your advisor to coordinate your schedule?
      \item To what degree did your advisor help or hinder your scheduling process?
    \end{itemize}

  \item Integrity items:
    \begin{itemize}
      \item How sincere did you find your advisor?
      \item How honest did you find your advisor?
      \item Based on the process and your ultimate course schedule, was your advisor just in their approach and outcome?
      \item How selfish was your advisor when constructing your schedule?
      \item Based on the process and your ultimate course schedule, was your advisor fair in constructing your schedule?
    \end{itemize}

  \item Benevolence items:
    \begin{itemize}
      \item How would you rate your advisor’s moral approach to your course scheduling?
      \item How would you rate your advisor’s ethical approach to your course scheduling?
      \item How would you rate your advisor’s sense of responsibility toward your academic goals?
      \item How considerate was your advisor throughout the process in regards to your goals and overall scheduling experience?
    \end{itemize}
\end{itemize}


\subsection{\citet{riedl2024patients} adapted trust measures}
\label{app:riedl-items}
\begin{itemize}
  \item Advisor Trust Items:
    \begin{itemize}
      \item The advisor is trustworthy.
      \item I have a good feeling when relying on the advisor.
      \item I can trust the information presented by the advisor.
    \end{itemize}

  \item AI Trust Items (shown only in AI-present conditions):
    \begin{itemize}
      \item The AI assistant is trustworthy.
      \item I have a good feeling when relying on the AI assistant.
      \item I can trust the information presented by the AI assistant.
    \end{itemize}

  \item Team Trust Items (advisor--AI team as a combined entity):
    \begin{itemize}
      \item The advisor-AI team is trustworthy.
      \item I have a good feeling when relying on the advisor-AI team.
      \item I can trust the information presented by the advisor-AI team.
    \end{itemize}
\end{itemize}

\subsection{Simulation Walkthrough}

\label{app:sim-walkthrough}


\begin{figure*}[htbp]
\centering
  % Row 1
  \includegraphics[width=0.47\linewidth]{figures/sim_shots/simintro.png}\hfill
  \includegraphics[width=0.47\linewidth]{figures/sim_shots/simshot1.png}
  
  \makebox[0.47\linewidth][c]{Step 1}\hfill\makebox[0.47\linewidth][c]{Step 2}

  % Row 2
  \includegraphics[width=0.47\linewidth]{figures/sim_shots/simshot2.png}\hfill
  \includegraphics[width=0.47\linewidth]{figures/sim_shots/simshot3.png}
  
  \makebox[0.47\linewidth][c]{Step 3}\hfill\makebox[0.47\linewidth][c]{Step 4}

\caption{Screenshots from a mistake simulation shown in chronological order (Steps 1--4).}
\label{fig:appendix-sim-seq}
\end{figure*}


\begin{figure*}[htbp]
\centering
% Row 3
  \includegraphics[width=0.47\linewidth]{figures/sim_shots/simshot4.png}\hfill
  \includegraphics[width=0.47\linewidth]{figures/sim_shots/simshot5.png}
  
  \makebox[0.47\linewidth][c]{Step 5}\hfill\makebox[0.47\linewidth][c]{Step 6}
  
  % Row 4
  \includegraphics[width=0.47\linewidth]{figures/sim_shots/simshot6.png}\hfill
  \includegraphics[width=0.47\linewidth]{figures/sim_shots/simshot7.png}
  
  \makebox[0.47\linewidth][c]{Step 7}\hfill\makebox[0.47\linewidth][c]{Step 8}

  % Row 5
  \includegraphics[width=0.47\linewidth]{figures/sim_shots/simshot8.png}\hfill
  \includegraphics[width=0.47\linewidth]{figures/sim_shots/simshot9.png}
  
  \makebox[0.47\linewidth][c]{Step 9}\hfill\makebox[0.47\linewidth][c]{Step 10}

  % Row 6
  \includegraphics[width=0.47\linewidth]{figures/sim_shots/simshot10.png}\hfill
  \makebox[0.47\linewidth]{} 
  
  \makebox[0.47\linewidth][c]{Step 11}\hfill\makebox[0.47\linewidth]{}

\caption{Screenshots from a mistake simulation shown in chronological order (Steps 5--11).}
\label{fig:appendix-sim-seq-part2}
\end{figure*}


==> Dennis-sections/cover_letter.tex <==
\pagenumbering{gobble}

\section*{Cover Letter}

Dear Program Chairs,

We thank the reviewers for their thoughtful and constructive feedback as well as the opportunity to revise our submission to address those critiques. We have updated the manuscript to address those concerns, including strengthening the theoretical positioning, engaging with more contemporary research relevant to our experiments, updating the experimental design and analysis, and clarifying the interpretation of results. Below, we summarize the key revisions and how they respond to the major critiques.

\begin{enumerate}
    \item \textbf{Alignment with FAccT and engagement with recent literature}

    To address concerns about positioning and relevance to FAccT, we significantly expanded the related work and theoretical framing. In particular, we now engage directly with recent FAccT literature on trust and reliance, including Kim et al. (2024) and Kim et al. (2023), and situate our work relative to these contributions. We clarify how our focus differs by examining workflow-level trust attribution under epistemic dependence, rather than reliance calibration in settings where correctness is independently verifiable. We also strengthen the connection to accountability and responsibility attribution in sociotechnical systems, making the contribution more clearly aligned with core FAccT themes.

    \item \textbf{Revised experimental design and analysis (factorial structure)}

    A central concern was the original five-condition design and lack of a fully specified factorial structure. In response, we restructured the study as a 3$\times$2 factorial design over advisor performance (error vs.\ no error) and AI intervention modality (none, proactive, reactive), including the previously missing no-AI error condition. We also increased the sample size (from $N=77$ to $N=157$) to support this design and conducted full factorial analyses. This revision directly addresses concerns about interpretability, clarity of factors, and statistical validity.

    \item \textbf{Clarification and calibration of claims}

    We revised the results and discussion sections to ensure that all claims are aligned with statistically supported findings. In particular:

    \begin{itemize}
        \item We now explicitly emphasize that advisor performance is the dominant driver of trust outcomes.
        \item We remove or soften claims about AI modality effects where statistical support is limited.
        \item We clearly distinguish between significant effects and descriptive trends.
    \end{itemize}

    These changes address concerns about overinterpretation and ensure that conclusions are appropriately scoped.

    \item \textbf{Strengthened the trust-to-reuse (reliance) connection}

    To address the ``so what'' critique regarding behavioral implications, we now explicitly frame trust as an evaluative judgment that governs reliance under uncertainty and connect it to downstream behavior via reuse intentions. This connection is now integrated into both the introduction and discussion, clarifying why trust differences matter for real-world decision-making and system adoption.

    \item \textbf{Improved clarity of design, measures, and presentation}

    We made several structural and clarity improvements throughout the paper:

    \begin{itemize}
        \item Reorganized hypotheses around the factorial design and reduced redundancy.
        \item Clarified experimental conditions, including how errors are surfaced to participants.
        \item Improved consistency in terminology (e.g., advisor vs.\ expert) and clarified the role of the user as the trustor.
        \item Provided clearer descriptions of measures, including the general trust item and reuse variable.
        \item Refined the discussion to better articulate the interpretation and limitations of findings.
    \end{itemize}

    \item \textbf{Refined contribution and interpretation}

    We revised the framing of the contribution to focus more precisely on trust attribution and responsibility within human-AI workflows. The paper now emphasizes that trust remains anchored to the human advisor even when AI visibly contributes, highlighting implications for accountability and system design rather than making overly strong prescriptive claims.
\end{enumerate}

We believe these revisions substantially strengthen the paper and address the reviewers’ concerns. Again, thank you for the time committed to our work and improving its construction.

\vspace{1em}
Sincerely,\\
Authors

==> Dennis-sections/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

This study examines how advisor performance and AI involvement shape trust judgments in an interactive academic advising task. The design allows us to distinguish performance-driven trust calibration from attributional effects associated with AI intervention modality.

\subsection{Trust Calibration to Performance and Modality}

Although all conditions produced a correct schedule, participants responded meaningfully depending on whether the advisor failed to detect an invalidating course choice. AI modality did not produce reliable factor-level effects, suggesting that perceptions of advisor performance were the most salient factor shaping trust evaluations. The observed pattern is consistent with prior work on trust calibration~\citep{Dzindolet2003Trust}, but in this setting these effects were concentrated on the human advisor rather than the AI assistant. 

The reuse-intention results extend this pattern from evaluative trust judgments to anticipated reliance behavior. Although we do not directly model the relationship between entity-specific trust and reuse, the parallel decline in reuse intention suggests that performance-related trust penalties may have downstream implications for continued reliance.  

Descriptive mean patterns suggest that AI involvement may shape evaluations in limited ways when errors are present, as performance-related declines followed a consistent ordering across modalities and multiple dependent variables, though these effects were not statistically significant at the factor level. Comparing average evaluation drops between errorless and error-present conditions generally showed the largest penalties in advisor-only workflows, followed by advisor-invoked AI workflows, and the smallest penalties under automatic AI oversight (Appendix~\ref{app:descriptive_tables}). These descriptive patterns suggest a possible avenue for future work: modality differences may become more salient in higher-stakes contexts, where advisor-invoked AI could signal uncertainty differently than automatic AI oversight.

Beyond mean differences, failure conditions were associated with greater variability in trust responses, with standard deviations consistently higher in error conditions than in their errorless counterparts, particularly for advisor-directed measures where Levene’s tests indicated significant differences. This pattern is detailed in Appendix~\ref{app:variance_tables}. This may reflect differences in how participants tolerate failure, the extent to which these errors violated expectations, or potential compounding effects from repeated errors. However, identifying the underlying driver of this pattern was not part of our experimental design and is left for future work. 

\subsection{Trust Attribution and the Effects of AI Involvement}

A central pattern in our results is that corrective AI changed the structure of the advisory workflow without significantly changing the target of trust consequences. Observed errors produced an attributional form of trust calibration, with trust consequences remaining anchored to the human advisor rather than being redistributed across the human-AI advisory system. Even when the AI assistant visibly detected and corrected errors, participants did not assign corresponding trust credit to the AI assistant. One interpretation is that AI correction creates a double signal: it demonstrates that the advisory workflow can recover from errors, but it also reveals that the human-facing advisor required correction. Under epistemic dependence, users may therefore treat the advisor as the primary bearer of responsibility, rather than crediting the AI assistant that contributes to the correction. In our setting, AI intervention modality defines how errors are detected and corrected, effectively acting as a governance mechanism over the advisory workflow. Across these modalities, verification authority is distributed differently. In advisor-only workflows, authority appears concentrated in the advisor; in proactive AI workflows, the advisor retains authority over when AI verification is invoked; and in reactive AI workflows, the AI assistant has more independent monitoring authority. However, changing this visible structure did not substantially redistribute trust among the advisor, the combined team, or the AI assistant alone. This interpretation is supported by the distribution of effects across trust targets in the measures adapted from \citet{riedl2024patients} (see Section~\ref{subsec:omnibus}).

One possible explanation is that users anchor trust judgments to the human interacting with the AI, consistent with work on algorithmic aversion showing that people may prefer human judgment over algorithmic judgment after observing imperfections, even when the algorithm performs well~\cite{dietvorst2015algorithm}. In our setting, however, the stronger effect was not distrust of the AI assistant but the absence of corresponding trust credit for its corrective role. Another potential explanation is that the AI corrected the error without providing indications of its own certainty. Unlike systems that explicitly communicate certainty levels~\cite{kim2024XAItrust}, our AI presented its correction without signaling how confident it was in that contribution. Participants may therefore have interpreted the AI’s role as procedural rather than judgment-based, giving them little basis for evaluating the AI’s independent trustworthiness. This may help explain why trust in the AI did not significantly change.

\textcolor{blue}{Relatedly, participants had limited evidence with which to evaluate the AI as an independent contributor. Because the AI assistant was always correct in the present study, participants never observed evidence of AI fallibility; at the same time, they were not given progressively deeper information about how the AI detected the problem, which evidence it used, or why its correction should be considered reliable. The stability of AI-directed trust should therefore be interpreted within a setting of perfect observed AI performance and limited transparency into the correction process, rather than as evidence that AI trust would remain unchanged under variable reliability or richer explanatory information. Work on progressive disclosure suggests that explanations can be revealed incrementally and on demand, allowing users to move from a high-level intervention cue to more detailed information without receiving all available detail at once (Muralidhar et al. 2025). Future studies could compare a simple correction notice with progressively disclosed information about the relevant rule, the AI’s reasoning, or its confidence to test whether the presentation of the correction changes how trust is attributed across the advisor, AI assistant, and advisor-AI team.}

These attributional patterns do not rule out a supportive role for AI in trust recovery. As discussed above, descriptive trends suggest that AI-supported workflows may modestly attenuate trust declines in error-present conditions (Appendix~\ref{app:descriptive_tables}). Although this pattern was not statistically significant, it warrants further study in higher-stakes settings or contexts where error transparency is nonnegotiable.

Taken together, these findings suggest a limit of procedural governance in human-AI advisory workflows. Altering who monitors, verifies, or corrects the workflow may not be sufficient to redistribute accountability when users rely on procedural cues under epistemic dependence. Instead, responsibility attribution remains concentrated on the human advisor, even when valuable contributions are more distributed across system components. This asymmetry may create an accountability burden for human experts in AI-assisted workflows: users may continue to assign responsibility to the human-facing advisor even when error detection and correction are distributed across the human-AI system.

\subsection{Implications for Human-AI Advisory Design}

Our results indicate that trust and reliance show similar patterns, with both general trust and reuse intention declining in error-present conditions (Appendix Table~\ref{tab:reuse_means}), suggesting that sustaining user trust is critical for promoting continued reliance on human-AI advisory systems. Because trust penalties were directed primarily at the human advisor, maintaining trust in the advisor should be a central focus for system design. The AI assistant received little to no direct trust credit, even when it contributed meaningfully to error detection and correction. 

For designers and institutions, this suggests that AI oversight should not be treated as automatically redistributing trust: users may continue to evaluate the human-facing expert as the primary responsible party even when AI support visibly shapes the final outcome.

Advisor performance emerged as the dominant factor shaping trust evaluations, with failures resulting in substantial declines in trust. Although an intuitive approach could include hiding errors, this is not always ethically or practically feasible, particularly in domains requiring nonnegotiable transparency. As a result, system design should assume that advisor errors may be observed and should focus on preserving perceptions of advisor competence and managing their impact.

For design, the descriptive ordering suggests that AI involvement may be most useful as a supportive safeguard rather than as a substitute for advisor competence. Even when AI assistance attenuates trust loss, it may not eliminate the penalty or shift responsibility away from the advisor. Automatic oversight may be especially useful in settings where advisor expertise is limited, but this possibility requires further empirical testing.

The greater variability observed after failures also has design implications: users may differ in how they interpret and tolerate advisor errors. One possible direction is to incorporate adaptive mechanisms that respond to user states of (dis)trust in real time, for example by adjusting the volume or quality of feedback provided following errors.

Taken together, these findings suggest that human-AI advisory design should prioritize advisor reliability while carefully structuring how AI participates in error detection and response. AI may play a supportive role in mitigating the impact of failures, but it should not be treated as a substitute for advisor competence or as a mechanism for redistributing responsibility.

\subsection{Generalizability and Broader Considerations}

Although situated in academic advising, our study reflects a broader class of expert-guided decision settings in which users lack the domain knowledge needed to independently verify correctness. Similar dynamics arise in financial advising, legal consultation, medical triage, and technical support~\cite{agrawal2023crosscultural, HanKo2025TrustDynamicsFA, mayer1995integrative, kaye2004roles}, where users evaluate experts based on observed performance.

The importance of these cues is likely domain-dependent. Higher-stakes, time-critical, longer-term, or more formally accountable settings may shift how users interpret failures, assign responsibility, and distribute trust across entities.

Although AI intervention modality did not produce reliable effects here, it may matter in other contexts. The present findings suggest that such effects are likely secondary to observed expert performance, especially when users directly witness failures.

More broadly, these results suggest that the experimental setup can capture meaningful variation in trust judgments and responsibility attribution within human-AI advisory workflows. This is reflected in entity-specific trust evaluations, including statistically significant performance-driven effects and measurable, though not statistically significant, differences across AI intervention modalities.

==> Dennis-sections/related-work.tex <==


\section{Relevant Work}

Research on trust in automation, human-AI interaction, and social epistemology
provides complementary perspectives that motivate our study design and trust
measurement strategy. This section organizes prior work around three questions central to our investigation:
(i) how trust responds dynamically to observed performance and error,
(ii) how procedural structure and responsibility cues shape trust in
AI-supported expert workflows, and (iii) how trust should be measured when
multiple potential trustees are present within a single interaction.



\subsection{Trust Calibration Under Epistemic Dependence}

A central theme in the trust-in-automation literature is that trust is not static, but evolves as users update their beliefs based on observed system behavior and outcomes~\cite{lee2004trust}. This process is especially important under epistemic dependence, where users cannot fully understand or independently verify system correctness and must instead rely on observable cues such as performance, communication, and interaction dynamics to calibrate trust~\cite{lee2004trust}. \textcolor{blue}{In this paper, trust recalibration refers to differences in participants’ reported trust judgments in response to observable evidence about advisor performance and AI involvement. Because trust was measured after a single between-subjects interaction, we operationalize recalibration as differences between error-present and errorless conditions rather than as within-participant change over time or as correspondence between trust and objectively measured reliability.} Recent work in human-AI interaction further formalizes trust in terms of user vulnerability and expectations over system behavior~\cite{jacovi2021formalizing}, while work on trust dynamics emphasizes that trust judgments emerge over interaction rather than from isolated assessments~\cite{HanKo2025TrustDynamicsFA}.

Empirical evidence reinforces that calibration operates at the level of individual interactions and outputs. For example, \citet{kim2023humans} show that users do not rely on AI systems with a fixed level of trust, but instead selectively accept or reject outputs after engaging in verification behaviors, highlighting the dynamic and context-sensitive nature of trust. Prior syntheses similarly emphasize that trust judgments depend on contextual factors such as task demands, perceived risk, and user expectations, and may diverge from objective performance metrics~\cite{hoff2015trust,Wong2025TrustAutomationAIHealthcare}. Work on AI-assisted ethical decision-making further shows that reliance on AI advice can vary with properties of the recommendation itself, including whether the recommendation reflects values aligned with the decision-maker~\cite{narayanan2023value}. Across domains, observed errors play a particularly important role in this process, as they provide salient evidence that can prompt users to update their beliefs about system reliability and competence. For example, work on algorithmic aversion shows that exposure to system errors can reduce subsequent reliance after users observe imperfections~\cite{dietvorst2015algorithm}.

Importantly, trust responses depend not only on whether an error occurs, but also on how that error is communicated and contextualized. \citet{Dzindolet2003Trust} demonstrate that feedback about system limitations and error characteristics enables more appropriate calibration, helping users avoid both overreliance and disuse. Work on AI communication similarly shows that factuality-expression formats can affect user trust in AI-generated answers~\cite{do2025hide}, while uncertainty-expression cues can modulate reliance by signaling limitations in system outputs~\cite{kim2024uncertainty}. Unlike settings where an AI system directly communicates reliability or uncertainty information to the user, our study examines AI assistance embedded within a human-facing expert workflow. In this setting, corrective AI may provide evidence of workflow-level recovery while also exposing the advisor’s need for correction, without necessarily making the AI assistant itself the primary target of trust. This motivates examining outcomes alongside how performance information is surfaced, interpreted, and attributed within an interaction.


Recent studies in AI-assisted advisory contexts further characterize trust as path-dependent and sensitive to sequences of interaction events. \citet{HanKo2025TrustDynamicsFA} show that salient errors can produce sharp declines in trust that may be partially repaired through subsequent corrective interactions, while \citet{Pareek2024TrustDevelopmentRepair} demonstrate that trust can propagate across stages of a workflow when users are able to evaluate some components but not others. These findings highlight that trust judgments are formed over trajectories of interaction, where both errors and corrective signals contribute to how responsibility and reliability are inferred over time.

Together, these studies position trust calibration as an interaction-level process shaped by observed outcomes, communicated performance information, corrective signals, and the user’s ability to evaluate what happened. This is especially important in epistemically dependent advisory settings. Building on this literature, our work examines whether trust judgments are shaped not only by final outcomes, but by whether the advisory workflow visibly encountered and resolved problems along the way, and by how AI support is incorporated into that sequence.

% \begin{figure*}[t]
%   \centering
%   \includegraphics[width=\textwidth]{figures/Fig2.png}
%   \caption{Interaction workflows for the academic advising paradigms examined in this study.}
%   \label{fig:workflows}
% \end{figure*}

\begin{figure*}[tbp]
  \centering
  \includegraphics[width=0.32\linewidth]{figures/adv_only_succ.jpg}\hfill
  \includegraphics[width=0.32\linewidth]{figures/initiated.jpg}\hfill
  \includegraphics[width=0.32\linewidth]{figures/automatic.jpg}
  
  \parbox[t]{0.32\linewidth}{(a)\label{fig:adv_only} $C_{adv\_only\_errorless}$ or $C_{adv\_only\_errors}$: advisor-only workflow without AI involvement.}\hfill
  \parbox[t]{0.32\linewidth}{(b)\label{fig:adv_ai_invoked} $C_{proactive\_errorless}$ or $C_{proactive\_errors}$: advisor-initiated AI assistance following a detected error.}\hfill
  \parbox[t]{0.32\linewidth}{(c)\label{fig:adv_ai_auto} $C_{reactive\_errorless}$ or $C_{reactive\_errors}$: automatic AI oversight that continuously monitors and intervenes.}
  
  \caption{Interaction workflows for the academic advising paradigms examined in this study.}
  \label{fig:workflows}
\end{figure*}

\subsection{AI Oversight, Workflow Governance, and Responsibility Attribution}

Beyond performance outcomes, trust judgments are also shaped by how users
interpret epistemic roles and responsibility within a workflow. In human-AI
settings, identical outcomes may support different inferences depending on
who appears to monitor, verify, and authorize decisions. \citet{YangMa2025EpistemicRelationships} argue that users’ evaluations of AI systems and AI-assisted decision-making contexts involve context-dependent assessments of epistemic authority, responsibility, system behavior, and underlying processes. A parallel distinction appears in formal work on AI trustworthiness: \citet{bisconti2024formal} distinguish the characteristics a system possesses from the characteristics observers infer from displayed behavior, and argue that perceived trustworthiness can depend on cues such as transparency, agency locus, and human oversight. In our setting, these process-based assessments are reflected through procedural cues in the
interaction (e.g., how AI intervention occurs).

Classic models of human-automation interaction similarly emphasize the
importance of procedural visibility. \citet{Parasuraman2000TypesLevelsAutomation}
note that higher levels of automation can obscure ongoing human involvement,
reducing users’ ability to distinguish between human and system contributions.
Such shifts do not inherently undermine trust, but they may alter how users
attribute responsibility for errors and corrections.

\textcolor{blue}{The amount and sequencing of information disclosed about AI involvement may also shape these attributions. Muralidhar et al. (2025) examine progressive disclosure as a transparency strategy in which explanations are revealed gradually and, in many cases, on demand rather than presented all at once. Their findings suggest that users value selectively presented explanations and that the order, modality, and technical complexity of those explanations affect perceived transparency and understanding. Applied to human-AI advisory workflows, this perspective suggests that trust attribution may depend not only on whether AI correction is visible, but also on how much information users receive about the correction process, when that information is presented, and whether they can request additional detail.}

Insights from social epistemology further suggest that trust is supported by
mechanisms that evaluate an informant’s competence and responsiveness to error
rather than by passive acceptance alone~\cite{Sperber2010EpistemicVigilance,Origgi2014EpistemicTrust}.
Observable signals of monitoring and correction can therefore function as
procedural evidence of epistemic responsibility. Related work on calibration
and credibility judgments shows that errors are particularly damaging when
they are interpreted as evidence of poor self-assessment rather than as
isolated outcomes~\cite{kim2004removing,tenney2008calibration,GriffinTversky1992}. Together, these perspectives motivate treating AI oversight as part of advisory workflow governance rather than as a purely technical aid. Our study builds on these perspectives by examining whether visible AI correction in a human-facing advisory workflow changes how trust consequences are allocated across the advisor, the AI assistant, and their combined operation, even when the final recommendation is correct.

\subsection{Trust, Reliance, and Accountability Across Multiple Targets}

A methodological challenge in AI-supported advisory systems is that a single
interaction may involve multiple plausible trustees. Users may evaluate the
human advisor, the AI system, and their combined operation differently, and
outcome evidence may not map cleanly onto a single target.



\citet{hendriks2015meti} conceptualize epistemic trustworthiness
as a multidimensional construct comprising expertise, integrity, and
benevolence, providing a validated framework for assessing trust in experts
under epistemic uncertainty. However, such measures alone do not capture how
trust is distributed across multiple entities when AI is involved. Prior work~\cite{riedl2024patients}
demonstrates that users can meaningfully provide entity-specific trust
judgments for human professionals, AI systems, and hybrid configurations
using parallel item structures.

This multi-target measurement strategy is central to our study. By separately measuring trust in the advisor, the AI assistant, and the advisor-AI team, we can test whether trust penalties and credit are allocated across specific components of the workflow or remain concentrated on the human expert despite visible AI involvement. \textcolor{blue}{We use trust consequences to refer to condition-related differences in trust evaluations and to the entities toward which those differences are directed. Operationally, advisor-directed trust consequences were assessed using epistemic trustworthiness, entity-specific trust in the advisor, and general trust. AI- and team-directed trust consequences were assessed using entity-specific ratings of the AI assistant and advisor-AI team in the AI-supported conditions. Likelihood of advisor reuse was analyzed separately as a behavioral proxy for anticipated reliance.}



==> Original-Sections/Results/analysis.tex <==
\subsection{Overview of Analytical Approach}
%Throughout this section, we distinguish between advisor-targeted trust,
%measured using the Riedl instrument, and global trust, measured using a
%single-item 1-100 scale.

For each trust construct, we conducted a one-way omnibus analysis of
variance (ANOVA) with condition as the independent variable. Outcomes
included METI expertise, integrity, and benevolence composites, an
additional aggregated trust measure adapted from prior work, a general
trust rating assessed on a 1-100 scale, and a behavioral intention measure
assessing participants’ likelihood of reusing the advisor. When an omnibus
test indicated a statistically significant effect, we followed with Tukey’s
HSD for post hoc pairwise comparisons. Effect sizes were estimated using
eta-squared ($\eta^2$) and Cohen's d, respectively. We report test statistics in standard ANOVA form
with exact degrees of freedom, and numerical values are reported alongside
the finalized analyses.

\subsection{Omnibus Tests Across Trust Constructs}
\srm{Add lines about what hypotheses is supported and not supported by each result}
ANOVA analysis revealed a significant effect of condition on perceived epistemic expertise, $F(4,\,\text{72}) = \text{2.86}$, $p = \text{0.03}$, $\eta^2 = \text{0.14}$. Descriptively, perceived expertise ratings were lowest in \reactfail, i.e, when the advisor asks for help from the AI system and it identifies a mistake. In post-hoc testing, \advonly\ was rated significantly higher than \reactfail.

In contrast, no significant differences across conditions were observed for the remaining METI dimensions of integrity and benevolence (all $p$s $> \text{0.05}$).

The Riedl et al. general trust measure also indicated a significant effect of condition on perceived trust in the advisor, $F(4,\,\text{72}) = \text{2.64}$, $p = \text{0.04}$, $\eta^2 = \text{0.13}$. 

There was also a significant effect of condition on participants’ reported likelihood of reusing the advisor, $F(4,\,\text{72}) = 3.43$, $p = .013$, $\eta^2 = \text{0.16}$.

No significant effects were observed for the general trust rating or for trust measures associated with AI-only or hybrid advisory conditions (all $p$s $> \text{0.05}$).

Across the constructs with significant differences, effect sizes were consistently medium (all $\eta^2$ in the .13–.16 range).

\subsection{Descriptive Statistics}
Table~\ref{tab:descriptives} reports descriptive statistics (mean $\pm$ SD) for trust constructs that exhibited significant omnibus effects: perceived epistemic expertise, aggregated trust, and likelihood of advisor reuse.

Across conditions, perceived expertise ratings were consistently lower in
workflows that contained scheduling errors than in workflows that resulted
in a correct schedule. A similar pattern was observed for aggregated trust
and likelihood of advisor reuse, with error-containing conditions evaluated
less favorably on average than successful advising workflows. 

These descriptive patterns are reported to contextualize the omnibus and post-hoc
tests reported below.


\begin{table}[t]
\centering
\caption{Descriptive statistics (mean $\pm$ SD) for key trust outcomes by condition.\textcolor{red}{Make the condition names consistent}}
\label{tab:descriptives}
\begin{tabular}{lccc}
\toprule
Condition & METI Expertise & Riedl Trust & Reuse \\
\midrule
\reactsucc       & 6.01 $\pm$ 1.11 & 6.00 $\pm$ 1.04 & 6.22 $\pm$ 1.11 \\
\reactfail       & 4.99 $\pm$ 1.57 & 4.90 $\pm$ 1.89 & 4.69 $\pm$ 2.12 \\
\advonly  & 6.36 $\pm$ 0.90 & 6.12 $\pm$ 1.35 & 6.36 $\pm$ 1.21 \\
\procsucc       & 6.01 $\pm$ 0.88 & 6.18 $\pm$ 0.79 & 6.00 $\pm$ 1.12 \\
\procfail      & 5.58 $\pm$ 1.27 & 5.56 $\pm$ 1.26 & 5.27 $\pm$ 1.62 \\
\bottomrule
\end{tabular}
\end{table}




\subsection{Pairwise Condition Comparisons}
For all Tukey HSD pairwise comparisons, mean differences are computed as
(condition$_2$ $-$ condition$_1$). Thus, negative values indicate higher
ratings in the first-listed condition.

Post-hoc pairwise comparisons were conducted for trust constructs that
exhibited significant omnibus effects. For perceived epistemic expertise,
Tukey HSD tests indicated that advisors in the adv\_only\_succ
condition were rated as significantly more expert than those in the
\texttt{init\_fail} condition (mean difference = \text{-1.37}, 95\% CI =
[\text{-2.67}, \text{-0.07}], $p = \text{0.03}$). No other
pairwise comparisons for expertise reached statistical significance.

For the aggregated trust measure, pairwise comparisons revealed that
participants rated the \procsucc condition as significantly more
trustworthy than the \reactfail condition (mean difference =
\text{-1.28}, 95\% CI = [\text{-2.55}, \text{-0.01}], $p =
\text{0.05}$). 

For likelihood of advisor reuse, Tukey HSD post-hoc tests indicated that reuse
intentions were significantly higher in the \advonly\ 
condition than in the \reactfail\ condition (mean difference
$= -1.68$, 95\% CI [$-3.31, -0.04$], adjusted $p = 0.04$). Reuse intentions were
also significantly lower in the \reactfail\ condition than in the
\reactsucc\ condition (mean difference $= 1.53$, 95\% CI
[$0.10, 2.97$], adjusted $p = 0.03$).

==> Original-Sections/Results/summary.tex <==
\subsection{Summary of Results}
Taken together, the results indicate that trust perceptions varied across
advising workflows in a manner primarily driven by advisory outcomes.
Workflows that contained scheduling errors were evaluated less favorably
than successful advising workflows across multiple trust-related measures,
including perceived epistemic expertise, entity trust, and likelihood
of advisor reuse. 
%\sout{Notably, reuse intentions do reinforce general trust sentiments, specifically when the advisor succeeds alone relative to when they make mistakes and must rely on AI voluntarily (reactive).}  
%\srm{I added this, double check} 
%\dk{I reworded yours earlier to this}
Notably, reuse intentions reinforce general trust in workflows characterized by advisory success rather than in workflows where the advisor fails to capture the invalidating issue, specifically in \advonly ~or \procsucc ~to \procfail. This is aligned with what we had originally expected (H7), where we assumed that reuse would be evident for setups where the advisor made no mistake. 
%To our surprise, manually-invoked AI (proactive) by the advisor resulted in lower expertise than in the reactive counterpart condition when the advisor failed to catch the mistake. This original expectation was borne out of the belief that proactive AI reflected both a lack of self-awareness on the advisor's part about potential mistakes and the fact that the AI proactively notifying the expert could potentially undermine the authority of the expert in the eyes of the end user.

No significant differences were observed for
integrity, benevolence, global trust, or trust judgments directed toward
AI-only or hybrid advisory entities.
At the same time, trust was not uniform amongst successful workflows. 
Across conditions without mistakes, mean trust ratings 
differed descriptively across AI integration configurations as expected. However, 
these differences were not statistically distinguishable at the current 
sample size ($N=77$), and no pairwise comparisons among successful 
conditions reached significance. These findings suggest that while performance
outcomes dominate trust judgments, the manner in which AI is integrated into
expert workflows can influence how users evaluate advisors and advisory
systems.

Interestingly, most of the significant pairwise comparisons on perceived expertise were absent of AI-involved workflows exclusive of scheduling issues, even though these conditions resulted in correct schedules. Significant contrasts were primarily confined to comparisons involving the advisor-only success condition and the proactive AI failure condition. Though this pattern is not conclusive, the absence of expertise differentiation among AI-assisted successes suggests that AI involvement may complicate or dampen expertise attribution, limiting the degree to which success alone enhances perceived competence. This contrast points to an intriguing avenue for future work on attribution and trust formation in AI-supported decision making.

==> Original-Sections/abstract.tex <==
AI systems are increasingly incorporated into professional workflows where
individuals traditionally rely on human experts, including domains such as
medicine, law, finance, and academic advising. As this shift accelerates, a
central question emerges: how does AI involvement shape users’ trust in the
human expert, the AI system, and their combination? To examine this, we
conducted an online advising study ($N=77$) in which participants completed
a simulated course-planning task that varied whether the advisor ultimately
produced a correct or incorrect schedule, and whether an AI assistant
intervened reactively (automatically) or proactively (only at the advisor’s invocation). A baseline
condition with a successful advisor and no AI involvement was also included.

After the interaction, participants rated trust using METI’s ~\cite{hendriks2015meti}
multidimensional epistemic trust axes, a willingness-to-reuse measure, and
entity-specific trust items targeting the advisor, the AI assistant, and
their combination ~\cite{riedl2024patients}. Results indicate that advisory outcomes strongly shape trust judgments, with error-containing workflows evaluated less favorably across a subset of measures gathered. Among workflows that achieved successful outcomes, trust ratings varied descriptively across AI integration configurations. While significant differences were detected for medium effects, smaller differences were not distinguishable with the current sample size. We discuss implications for designing human–AI advisory workflows, highlighting how procedural visibility and responsibility cues may influence trust even when outcomes are correct.

==> Original-Sections/discussion.tex <==






\section{Discussion}
\label{sec:discussion}

This study examined how trust judgments form in response to different patterns of advisor performance and AI involvement within an interactive academic advising task. By operationalizing each condition as a complete advising workflow - rather than isolating performance and AI involvement as independent factors - our design captures how such systems are likely to be encountered in practice.

\subsection{Trust Calibration to Observed Performance}
Consistent with prior work on trust calibration \citet{Dzindolet2003Trust}, the findings indicate that
participants’ trust judgments were strongly shaped by observed advisory
outcomes. Advising workflows that resulted in correct schedules were
evaluated more favorably than workflows that contained scheduling errors
across multiple trust-related measures.

Importantly, we can identify a worst-performing workflow on the outcomes
for which condition effects were detectable. Across perceived epistemic
expertise, advisor trust, and likelihood of advisor reuse, the
\procfail\ condition was evaluated most negatively for the advisor, and it was the
primary driver of the significant omnibus effects and the significant
post-hoc contrasts reported in Section~\ref{sec:results}. The \reactfail\
condition was also descriptively lower than the successful workflows, but
these differences were less consistently distinguishable in pairwise tests
at the current sample size.

Interestingly, this penalty was specific to the advisor-initiated failure condition.
Although both \reactfail\ and \procfail\ involved observed advising
errors, only \procfail\ produced significant reductions in advisor expertise,
aggregated trust, and reuse intention relative to successful workflows. The absence of
comparable penalties for \reactfail\ suggests that the mode of AI intervention,
not failure alone, shaped how trust consequences were allocated.

One interpretation is that visible advisor-initiated consultation following an error
may signal insufficient competence or poor calibration, whereas automatic oversight
allows error correction without directly implicating the advisor’s epistemic judgment.
As a result, participants may have attributed responsibility for failure more strongly
to the advisor in \procfail\ than in \reactfail, despite similar
outcome structure.


At the same time, trust judgments were not reducible to outcome success
alone. Among workflows that produced correct schedules, differences in how
AI involvement was introduced were associated with distinct trust patterns
across epistemic and behavioral measures. However, these differences did
not reach statistical significance among successful conditions at $N=77$,
suggesting that any within-success effects of AI configuration are more
subtle than the penalty associated with an observed advising error.

\subsection{Differentiation Among Successful Advisory Workflows}
Although advisory outcomes exerted a dominant influence on trust judgments, 
trust was not uniform across successful workflows. Differences across AI 
integration configurations were observable at the descriptive level, but 
did not reach statistical significance in the present study. This pattern suggests that users may attend to procedural differences in how 
AI support is integrated into the advising process, though detecting these 
effects reliably may require greater statistical power or repeated exposure.

Importantly, these differences did not reflect a reversal of outcome-based
trust calibration. Rather, they suggest that once a baseline of successful
performance is established, users may attend to additional cues - such as the
visibility of advisor judgment or the locus of corrective authority - when
forming trust judgments. This interpretation aligns with accounts of trust
as a multidimensional evaluation shaped by both outcomes and interactional
structure.


\subsection{Implications for Human-AI Advisory System Design}

Whether AI oversight is automatic, advisor-initiated, or absent altogether provides participants with potential cues about responsibility, competence, and accountability within the advising process. Trust may be shaped not only by whether failures occur, but by how responsibility, correction, and AI involvement are communicated and enacted during interaction.

Designers should therefore consider advising workflows holistically, accounting for how performance outcomes and AI intervention patterns jointly shape user trust over the course of interaction.

\subsection{External Validity and Generalizability}

Although the present study is situated in an academic advising context, the 
interactional structure examined here is representative of a broader class 
of expert-guided decision-making workflows in which users lack sufficient 
domain knowledge to independently verify correctness. Similar dynamics arise 
in domains such as financial advising, legal consultation, medical triage, 
and technical support, where individuals rely on expert judgment that may be 
augmented or overseen by AI systems. In such settings, users often evaluate 
trust not only based on outcomes, but also based on observable cues about how 
expertise, monitoring, and correction are enacted during the interaction. 
Accordingly, the workflow-level trust dynamics observed in this study may 
generalize to other human-AI advisory contexts in which epistemic 
responsibility and correction authority are distributed across human and AI 
components.

At the same time, several aspects of the present findings are likely to be 
domain-dependent. Academic advising involves moderate stakes, limited time 
pressure, and relatively transparent success criteria compared to domains 
such as medicine or financial decision-making, where errors may carry 
significant personal or economic consequences. In higher-stakes or 
time-critical settings, outcome failures may exert a stronger influence on 
trust judgments, potentially overwhelming more subtle procedural cues. 
Additionally, longer-term relationships, repeated interactions, or formal 
accountability structures may alter how users interpret AI involvement and 
expert responsibility over time. These considerations suggest that while the 
workflow-oriented perspective on trust formation is broadly applicable, the 
relative weighting of outcomes versus procedural signals may vary across 
domains and use cases.

\subsection{Broader Impacts, Harms, and Stakeholders}

The findings of this study have implications for the design and governance of 
AI-assisted advisory systems beyond individual user experience. In particular, 
they speak to how accountability, responsibility attribution, and transparency 
are negotiated when advisory outcomes are produced through human-AI 
collaboration. When AI systems are integrated as oversight or corrective 
mechanisms, the visibility of who initiates checking, detects errors, or 
authorizes corrections may influence how users assign epistemic responsibility 
to human advisors versus automated systems. Poorly designed workflows risk 
obscuring accountability, enabling blame shifting between human and AI actors 
following errors, or fostering misplaced trust in systems whose corrective 
roles are not well understood by users.

These dynamics also raise concerns about overreliance and underreliance. If AI 
oversight is framed as automatic or infallible, users may discount the human 
advisor’s role entirely or assume that errors are always prevented, increasing 
the risk of overtrust. Conversely, opaque or inconsistently applied AI 
interventions may undermine confidence in both the advisor and the system, 
leading to disuse even when performance is reliable.

From a stakeholder perspective, the consequences of these design choices extend 
to multiple groups. End users may benefit from advisory workflows that clearly 
signal responsibility and competence, but may be harmed by systems that mask 
error sources or shift blame inappropriately. Human advisors may experience 
erosion of perceived expertise or authority if AI involvement is framed in ways 
that diminish their epistemic agency, while institutions deploying such systems 
may face governance and liability challenges if responsibility boundaries are 
unclear. These considerations underscore the need for trust-sensitive design 
approaches that explicitly account for how AI integration shapes accountability 
relationships, rather than treating AI assistance as a purely technical 
augmentation.


==> Original-Sections/hypotheses.tex <==
\section{Hypotheses}
\label{subsec:hypotheses}
To examine how advisor performance and AI involvement shape students’ trust in our advising interaction, we formulated three hypotheses corresponding to the five experimentally varied conditions. These conditions combine advisor success or failure with either no AI assistance, reactive AI intervention, or proactive AI invocation by the advisor. Because our analysis compares trust across these five conditions using a one-way ANOVA followed by conditional pairwise comparisons, hypotheses are expressed as predicted differences in mean trust between conditions.

Accordingly, the tests reported below evaluate whether the workflows produce distinguishable trust profiles, and whether the direction of those differences aligns with the qualitative expectations described in H2-H3.

The hypotheses were motivated by intuitive expectations about how users interpret success, failure, and AI involvement in expert-guided interactions. Prior work on trust in automation suggests that observed failures serve as salient signals that prompt trust recalibration, particularly when users rely on an expert rather than verifying correctness themselves. We therefore expected workflows containing errors to produce lower trust in the advisor (H2). Among successful workflows, we anticipated that AI modality would alter perceived responsibility for the outcome. In particular, proactive AI consultation by the advisor was expected to signal uncertainty or reduced advisor competence relative to reactive oversight or no AI involvement, leading to lower trust in the advisor even when outcomes were correct (H3). This distinction aligns with accounts of human-automation interaction that emphasize how agency and initiative are distributed within a workflow. In Parasuraman et al.’s framework, differences in who initiates monitoring and verification reflect different allocations of decision authority, which can influence how observers interpret an expert’s epistemic responsibility even when task outcomes are identical. Finally, given these differing interaction dynamics, we expected trust to vary across the full set of workflows rather than remaining uniform (H1).


\subsection{Tested Hypotheses}
\label{}

The hypotheses below concern differences in trust judgments across the five experimental conditions, each of which corresponds to a distinct advising workflow (see Fig.~\ref{fig:workflows} for condition illustrations).

\begin{itemize}
    \item H1: Mean trust will differ significantly across the five conditions for
    aggregated trust measures.

    \item H2: Trust in the advisor will be lower in advising workflows that contain
    an error than in workflows that result in a correct schedule. Specifically:
    \begin{itemize}
        \item H2a: Trust in the advisor will be lower in the advisor-initiated failure
        condition ($C_{init\_fail}$) than in all success workflows.
        \item H2b: Trust in the advisor will be lower in the automatically corrected
        failure condition ($C_{auto\_fail}$) than in all success workflows.
        \item H2c: Trust in the advisor will be lower in the reactive AI condition ($C_{auto\_fail}$) than in the proactive AI condition ($C_{init\_fail}$).
    \end{itemize}


    \item H3: Among conditions in which the advisor produces a correct schedule,
    trust in the advisor will be lowest when the advisor proactively consults AI
    (manual invocation), higher under reactive (automatic) AI supervision, and
    highest when no AI is involved.
\end{itemize}

These hypotheses were specified a priori as directional expectations about how the failure and correction modality would influence trust. As reported below and in Section~\ref{sec:results}, some outcomes did not align with these expectations.

Overall, the hypotheses received mixed support. H1 was partially supported, as epistemic trust measures showed only marginal differences across conditions (p=.0539). H2 was partially supported, as advisory failure was associated with lower trust in the human advisor and reduced willingness to reuse only in the proactive AI failure condition, while automatic failure correction did not produce significantly lower trust relative to other workflows. H3 was not supported, as trust in the advisor did not differ significantly among successful conditions based on whether AI assistance was proactive, reactive, or absent. We treat these deviations from the a priori expectations as theoretically informative, highlighting the dominant role of observed advisor failure, rather than correction modality alone, in shaping trust judgments.

==> Original-Sections/intro.tex <==
\section{Introduction} 
Across domains such as healthcare, financial advising, legal consultation, and others, people depend on human experts to help them navigate complex decisions. Trust in these experts forms the foundation of these interactions. As AI systems increasingly enter these workflows, it expands the locus of control from a single expert to a constellation of contributors in producing guidance. Importantly, the mere presence of an AI system - independent of its specific behavior - may color users’ perceptions of trust, reshaping how users interpret responsibiity and credibility within the advisory process. From an epistemic trust perspective, these perceptions can be decomposed into
distinct judgments about an advisor’s expertise, integrity, and
benevolence~\cite{hendriks2015meti}. In our setting, advisory success or failure
directly provides evidence about perceived expertise (competence to satisfy constraints),
while the timing and visibility of AI oversight can introduce cues that affect integrity-
and benevolence-related inferences (e.g., whether the advisor appears transparent,
careful, and oriented toward the student’s best interest). Understanding how AI involvement affects trust in each of these elements is essential at a moment when AI integration is accelerating. In this work, we focus on a specific form of AI integration: AI systems that provide oversight by intervening either reactively - automatically monitoring and flagging issues - or proactively, when invoked at the human advisor’s discretion. We examine how these different forms of AI assistance shape users’ trust judgments in expert-guided interactions.

Prior work has examined trust in algorithmic systems \cite{lee2004trust,lee2018understanding} and trust in human experts \cite{hendriks2015meti}, but much less is known about how trust forms and changes when both entities contribute to a precision-dependent task, particularly how users interpret when and why AI systems intervene. If the advisor fails to detect an error and the AI identifies it, the interaction creates a moment in which users may reconsider prior assumptions about the source of guidance involved in the interaction. In particular, we examine how proactive versus reactive AI assistance affects trust when AI oversees expert workflows. Understanding these effects is critical for designing human-AI systems that support such workflows without undermining trust. Importantly, such moments require users to analytically distinguish trust directed towards the advisor, AI, and the configuration as a whole, each of which may be evaluated differently depending on how and when AI intervention occurs.

Advising workflows naturally support both proactive AI assistance, such as automatic detection of violations, and reactive assistance, such as advisor-initiated checks following changes, making them well suited for examining how intervention timing and visibility affect trust. As advising workloads grow and complexity increases, institutions have begun integrating AI tools to navigate degree requirements, support course-planning decisions, and more \cite{edutechloft2025_student_advising}. These developments raise a central question: how does the timing and visibility of AI assistance shape users’ trust in the advisor, the AI system, and their collaboration?

Importantly, the workflow conditions we study are not merely ``AI present vs.\ absent,''
but different epistemic cue profiles in Hendriks et al.’s sense~\cite{hendriks2015meti}.
For example, when an advisor succeeds without AI (\texttt{adv\_only\_succ}), the interaction
provides a strong competence cue. When the advisor
invokes AI proactively (\texttt{init\_succ}), that visible consultation may be interpreted
either as diligence (supporting integrity/benevolence) or as reduced competence (lower
expertise), even when outcomes are correct. When an error occurs and is corrected only
after the advisor initiates checking (\texttt{init\_fail}), the error itself can reduce
expertise while the invoked AI confirmation may additionally affect integrity-related
inferences about carefulness and reliability. In contrast, automatic oversight
(\texttt{auto\_fail}) can shift
attributions of expertise away from the advisor and toward the AI, reshaping how
participants distribute epistemic trust across the advisor, the AI, and the team.

To investigate these questions, we conducted a controlled online academic advising simulation that explicitly manipulates AI intervention strategy, including no AI assistance, proactive oversight, and reactive oversight, alongside advisor performance defined by success versus failure. Participants then rated their epistemic trust in each entity individually, namely the advisor, the AI assistant, and the advisor-AI team, as well as their general judgments of trustworthiness. This design allows us to examine how intervention shapes trust in those entities.

Academic advising offers a representative environment for studying these dynamics. Advisors must interpret degree requirements, identify prerequisite constraints, and ensure that course selections satisfy institutional policies, tasks that require specialized knowledge. At the same time, the stakes of advising are moderate enough that trust can be studied without the confounders present in riskier domains such as medicine or finance. 
 

Our results show that advisory outcomes are the primary driver of trust-related consequences, with conditions involving errors evaluated less favorably across multiple measures. In particular, advisory failure significantly reduces willingness to reuse the advisor or system and undermines perceptions of advisor epistemic expertise selectively as well as general trust. These effects are not uniform across trust targets, as material differences emerge primarily in evaluations of the human advisor, while trust in the AI system and the human-AI team remains comparatively equal. Together, these findings indicate that while success or failure affects overall trust judgments, AI involvement shapes where trust consequences are borne following advisory errors.

\subsection{Contributions}
\label{subsec:contributions}

This paper makes three contributions:
\begin{enumerate}
    \item We present an interactive, workflow-level experimental setup for
    studying trust in human-AI advisory systems that enables separate trust
    judgments about the human advisor, the AI assistant, and their combined
    operation under controlled performance and integration configurations.

    \item Using this setup in an academic advising task ($N=77$), we provide empirical
    evidence that advisory outcomes are a primary driver of trust-related evaluations,
    while also suggesting that proactive versus reactive AI assistance can shape trust judgments even when advisory outcomes are successful.

    \item We derive design implications for human-AI advisory workflows, emphasizing the role of intervention timing, procedural visibility, and perceived responsibility (e.g., who initiates
    checking or correction and how that role is surfaced) in structuring users’ trust in
    the advisor, the AI, and the advisory team.
\end{enumerate}



==> Original-Sections/limitations.tex <==
\subsection{Limitations}
We took care in designing this simulation to approximate a realistic, though necessarily simplified, interaction involving AI-supported decision-making. Nevertheless, several limitations should be acknowledged. First, the use of a between-subjects design prevents individual participants from directly comparing different advising interactions or outcomes, which may limit insight into how trust recalibrates across repeated interactions.

As with all controlled experimental studies, the findings may also be limited in their generalizability beyond the simplified advising task, interface, and population studied. While we sought to enhance situational validity through a realistic advising scenario and grounded operationalizations of advisor performance and AI involvement, participants’ perceptions may differ in real-world advising contexts and especially in higher-stakes expert domains such as medicine, legal consultation, or finance. We therefore interpret the present results as evidence about trust attribution under conditions of epistemic dependence in a controlled proxy setting, rather than as a direct estimate of how strongly the same effects would appear in safety-critical environments.

\textcolor{blue}{A further limitation is that the AI assistant was always correct when it intervened. This design allowed us to isolate the effects of advisor performance and AI intervention modality, but it does not capture settings in which AI assistance may itself be uncertain, incorrect, or inconsistently reliable. Participants therefore had no evidence from which to evaluate the consequences of AI failure, which may have limited variation in AI-directed trust ratings and contributed to the absence of significant effects for trust in the AI assistant. Future work should vary AI reliability and examine how advisor errors and AI errors jointly shape trust in the advisor, the AI assistant, and the human-AI team.}

Additionally, individual differences such as prior experience with academic advising, familiarity with AI systems, or general attitudes toward automation may have influenced trust judgments. These factors were not explicitly measured and therefore fall outside the scope of the present study. Future work could examine how such individual characteristics interact with advisor performance and AI involvement to shape trust, including whether they moderate which aspects of trust are affected and which remain stable.

Although our results suggest that responsibility attribution remained anchored to the human advisor, we infer this pattern from the distribution of trust judgments across the advisor, AI assistant, and advisor-AI team rather than from a direct measure of perceived responsibility or accountability. Future work should include explicit responsibility-attribution measures to test this interpretation more directly.

==> Original-Sections/measures.tex <==
\subsection{Measures}
\label{subsec:measures}

We intentionally employed multiple trust measures to capture distinct but complementary aspects of trust in human-AI advisory interactions. The \citet{hendriks2015meti} instrument was used to assess epistemic trustworthiness in the advisor, while items adapted from \citet{riedl2024patients} captured broader entity-specific trust judgments toward the advisor, AI assistant, and advisor-AI team. Consistent with \citet{lee2004trust}, these items capture trust as an evaluative attitude toward system entities. Finally, the single-item trust measure provided a holistic assessment of trust that was not decomposed into specific dimensions, allowing us to examine whether broader trust judgments aligned with or diverged from measures of specific characteristics.

Items were drawn from these prior works~\cite{hendriks2015meti,riedl2024patients} and adapted to the academic advising scenario through minor wording changes when necessary (e.g., replacing domain-specific referents with ``advisor,'' ``AI assistant,'' or ``advisor-AI team'') while preserving the original response formats and construct intent. Unless otherwise noted, all multi-item measures were assessed using a 7-point Likert scale ranging from 1 (``Strongly [disagree/negative
construct]'') to 7 (``Strongly [agree/affirmative construct]''). Questionnaire
items from~\citet{riedl2024patients} and~\citet{hendriks2015meti} used in the study are reported in Appendices~\ref{app:riedl-items} and~\ref{app:meti-items}, respectively.

For multi-item constructs, we aggregate items within each instrument’s intended structure and report results at the composite level when appropriate. This approach reduces item-level noise and aligns inference with the theoretical level at which the constructs are defined (e.g.,~\citet{hendriks2015meti} expertise, integrity, and benevolence), while preserving the original response scale as originally structured. In addition, aggregating items according to validated instrument structures \cite{hendriks2015meti} reduces the number of statistical tests performed, thereby limiting family-wise error rate (FWER) inflation and the risk of spurious significance.

\subsubsection{Epistemic Trustworthiness (METI)}

To assess participants’ epistemic trust in the advisor, we administered items from the Muenster Epistemic Trustworthiness Inventory (METI)~\cite{hendriks2015meti}. METI operationalizes epistemic trustworthiness along three dimensions: perceived expertise, integrity, and benevolence, reflecting perceived competence, adherence to professional standards (e.g., honesty and fairness), and goodwill toward others, respectively. Following the instrument’s dimensional structure, we computed dimension scores by averaging item responses within each dimension (higher scores indicate stronger perceived epistemic trustworthiness). Item counts and internal consistency for each composite are reported in Appendix~\ref{app:measures}. The full METI item set and dimension groupings used in this study are provided in Appendix~\ref{app:meti}.

\subsubsection{Trust in the Advisor, AI System, and Team}

In addition to epistemic trustworthiness, we measured entity trust using three items adapted from \citet{riedl2024patients}. \textcolor{blue}{Items were reformulated to fit the academic advising scenario. All participants completed items targeting the advisor, while participants in the AI-supported conditions additionally completed parallel items targeting (i) the AI assistant and (ii) the advisor-AI team as a combined advisory entity. Participants in the advisor-only conditions did not rate the AI assistant or advisor-AI team because those entities were not present in their assigned workflow.} An example item is: ``I can trust the information presented by the advisor.''  
All items demonstrated acceptable internal consistency as measures of entity trust (see Appendix~\ref{app:measures}).

\subsubsection{General Trust}

To capture a global assessment of trust that was not tied to a specific Likert instrument, participants completed a single-item general trust rating: ``From 1-100, how trustworthy would you rate your advisor? (1 being the least trustworthy and 100 being the most)''. This measure served as a holistic outcome capturing overall trust in the advisor unconstrained by specific item framing. A continuous scale was used to allow for finer-grained variation in global trust judgments than would be possible with a coarse Likert scale.

\subsubsection{Likelihood of Advisor Reuse}

To assess behavioral intention, participants reported their likelihood of reusing the advisor in the future. This single-item outcome was analyzed separately from the multi-item trust composites.

We treat reuse intention as a behavioral proxy rather than as a direct trust measure. Whereas trust instruments capture evaluative judgments (e.g., perceived expertise or trustworthiness), reuse intention reflects whether participants would act on those judgments by relying on the advisor again. Reuse intention is particularly relevant in advisory settings, where the practical consequence of trust is often continued reliance over time. Including this measure, therefore, allows us to assess whether differences in epistemic trust or entity-level trust correspond to differences in anticipated reliance on the advisor.

==> Original-Sections/participants.tex <==
\subsection{Participants}

Participants were recruited through Prolific~\cite{prolific} and completed the study remotely. Repeat participation was systematically restricted using Prolific’s built-in eligibility controls to maintain data integrity. Participation was restricted to desktop or laptop users to ensure consistent interaction with the advising interface. In addition, participants were excluded from analysis if they failed the attention-check questions embedded throughout the study, including within the interactive simulation and the final questionnaire. No other exclusion mechanisms were applied. 

A total of 160 participants completed the study. After accounting for those failing the attention-checks, the final analytic sample was $N = 157$. Each was compensated \$4.50 for their time upon completion of the study. All study procedures were approved by the institutional review board, and informed consent was obtained from all participants. Participants were assigned to experimental interactions via Prolific’s randomization, and demographic information is summarized in the Appendix~\ref{app:participant-breakdowns}. The study took approximately 17 minutes to complete, including the advising simulation and post-task questionnaire.

==> Original-Sections/related-work.tex <==
\section{Relevant Work}

Prior research across trust in automation, human-AI interaction, and social
epistemology provides complementary perspectives that motivate the design of
our study and the structure of our trust measurements. Rather than organizing
this literature paper by paper, we group relevant contributions according to
how they inform three aspects of our investigation: (i) trust as a dynamic
response to observed performance and error, (ii) how procedural structure and
responsibility cues shape trust in expert workflows that include AI, and
(iii) how to measure trust when multiple potential trust targets are present
within a single interaction. This organization clarifies the conceptual
assumptions behind our workflow-level manipulations and supports interpreting
how participants distribute trust across the advisor, the AI assistant, and
the advisor-AI team.

\subsection{Trust as Dynamic and Performance-Contingent}

A foundational theme in the trust-in-automation literature is that trust is
not a fixed trait or stable preference, but an evaluative judgment that
governs reliance under uncertainty and vulnerability. Lee and See
\cite{lee2004trust} frame trust as a mediator of reliance
decisions, emphasizing that users draw inferences from observed behavior and
that these inferences can diverge from objective accuracy \cite{lee2018understanding}. In this view,
trust should be studied as something that shifts as interaction unfolds,
especially when users cannot easily verify correctness and must instead
interpret cues from outcomes and process.

Related syntheses reinforce that trust judgments are sensitive to context,
including task demands, perceived risk, and user expectations, and that
perceived trustworthiness can differ from formal performance metrics
\cite{Wong2025TrustAutomationAIHealthcare}. Across application domains,
observed errors are commonly treated as salient interactional events because
they provide concrete evidence, triggering reassessment. However, this
does not imply that trust shifts are irrational or uniform across settings.
Rather, the reviews motivate careful attention to the interaction context in
which performance information is encountered, including what users believe
they are entitled to expect from a system or expert in that domain.

Empirical work on automated decision aids further suggests that trust and
reliance depend not only on whether an error occurs, but also on how the
error is surfaced, contextualized, and addressed. Dzindolet et al. ~\cite{Dzindolet2003Trust} show that feedback about limitations and error characteristics can support more appropriate calibration, helping users avoid both overreliance and disuse. While \citet{Dzindolet2003Trust} focuses on automated aids, it provides a useful mechanism-level motivation for studying advisory workflows as sequences of events, rather than as static treatments. In advisory
contexts, users often encounter a bundle of cues, including success, failure, and corrective feedback, and may update trust based on that bundle.

Recent work in AI-supported advisory settings similarly characterizes trust
as path-dependent and sensitive to error exposure, while also emphasizing
that trust need not remain permanently reduced after an error. Han and Ko
\cite{HanKo2025TrustDynamicsFA} examine trust dynamics in financial advisory
settings and highlight that a salient error can produce a sharp decline, and
that subsequent repair attempts can partially restore trust. Pareek et al.
\cite{Pareek2024TrustDevelopmentRepair} also emphasizes that trust can propagate
across stages of a workflow when users can verify some parts but not others,
and that repair framing can influence post-error trust even under identical
performance. Together, these results motivate studying trust as an outcome
shaped by concrete episodes of success, failure, and correction, and they
support designs that compare trust across complete workflows that differ in
performance and in how correction is initiated and communicated.

In the present study, these ideas motivate two choices. First, we treat the advisor’s failure to detect a task-preventing issue within the advising workflow as a primary informational event that can plausibly drive trust recalibration when participants are unable to independently verify correctness. Second, we treat AI involvement not as
a background feature, but as part of the interaction sequence that may affect
what participants infer from performance evidence. This framing supports
comparing trust across workflows that differ in error exposure and in the
structure of corrective oversight.

\subsection{Procedural Cues, Epistemic Roles, and Responsibility in Human-AI Workflows}

Although performance outcomes are central, a separate line of work emphasizes
that trust judgments can also reflect how users interpret epistemic roles and
responsibility within a workflow. 
In human-AI settings, the same observable
outcome can plausibly support different inferences depending on who appears
to monitor, verify, and authorize key steps. Yang and Ma
\cite{YangMa2025EpistemicRelationships} develop the notion of epistemic
relationships, arguing that evaluations of AI systems include judgments not
only about accuracy, but also about epistemic authority, responsibility, and
appropriateness in context. This perspective motivates examining trust as a
judgment that can be shaped by role structure and by cues that signal how
knowledge claims are generated and checked.

Classic models of human-automation interaction similarly highlight the
importance of procedural visibility for how users interpret agency and
accountability. Parasuraman et al. \cite{Parasuraman2000TypesLevelsAutomation}
distinguish levels of human involvement across stages of processing, and note
that higher automation can reduce the visibility of ongoing human engagement.
When monitoring or verification is automated, users may have fewer cues for
understanding what the human did, what the system did, and how errors were
detected. This does not imply that automation is inherently harmful to trust,
but it suggests that changing how oversight occurs may change what users
attribute to each actor.

Insights from social epistemology provide additional grounding for why these
procedural cues might matter. Epistemic vigilance characterizes trust as
supported by mechanisms that evaluate an informant’s competence, honesty, and
responsiveness to error, rather than by passive acceptance alone
\cite{Sperber2010EpistemicVigilance}. In this framing, trust can be sustained
by observable signals of monitoring and correction, because such signals
provide evidence that an agent is engaging in epistemic responsibility. This
motivates designs that vary whether checking and correction are visible and
how they are initiated, since those features plausibly affect what users
infer about competence and responsibility.

Work on calibration and credibility judgments further sharpens this point by
distinguishing error per se from what errors imply about an agent’s
self-assessment. Tenney et al. \cite{tenney2008calibration} show that
credibility judgments depend on perceived calibration, meaning whether a
source appears to know the limits of their knowledge and to regulate
confidence appropriately. Under this view, errors can be especially damaging
when they are interpreted as evidence of poor calibration, not merely as
unfortunate outcomes. This is relevant to workflows in which an error is
revealed and then corrected, because the correction episode can supply cues
about whether the agent noticed the issue, whether the agent anticipated the
risk, and whether the agent relied on an appropriate checking process.

Related evidence on confidence formation suggests that people often rely on
qualitative cues about evidential strength, rather than on normative weight,
when forming confidence judgments. Griffin and Tversky
\cite{GriffinTversky1992} show that confidence can be driven more by the
perceived strength or coherence of the evidence than by its statistical
warrant. In advisory interactions, this implies that observable signals of
deliberation, checking, or verification may shape perceived competence even
when those signals do not directly change the final outcome. This does not
require assuming that participants make explicit statistical inferences.
Rather, it motivates treating procedural features as inputs to the
impressions participants form about competence and responsibility.

Origgi’s account of epistemic trust as a procedural stance further supports
this emphasis on process. Origgi \cite{Origgi2014EpistemicTrust} describes
epistemic trust as a rational procedure for extracting information from
others while maintaining epistemic agency. In this view, trusting is
compatible with continued evaluation of coherence, competence, and
motivations, and trust can be revised as interaction unfolds. This aligns
with the idea that workflow structure matters, because it changes what
procedural evidence is available for users to update their stance. In
particular, visible checking or correction can serve as procedural evidence
that informs judgments about epistemic agency and responsibility.

Taken together, these frameworks motivate examining AI oversight as a
procedural feature that can shape how responsibility is perceived and how
trust consequences are allocated. They also motivate interpreting differences
between reactive and automatic oversight in terms of what those modes imply
about who is epistemically responsible for noticing and addressing problems,
without assuming any single fixed interpretation across all participants.

\subsection{Measuring Trust in Expert-Guided, Multi-Entity Contexts}

A key methodological challenge in human-AI advisory systems is that a single
interaction can involve multiple plausible trustees. Users may evaluate the
human advisor, the AI assistant, and the combined advisory configuration in
different ways, and outcome evidence may not map cleanly onto a single target.
This motivates trust measurement approaches that are sensitive to both the
dimension of trust being assessed and the entity to which it is directed.

Hendriks et al. \cite{hendriks2015meti} conceptualize epistemic
trustworthiness as a multidimensional judgment that supports deference under
epistemic uncertainty. Their METI framework distinguishes expertise,
integrity, and benevolence as separate evaluative dimensions. This structure
is especially relevant to expert-guided tasks where participants are not
expected to verify correctness directly. In such settings, trust judgments
often reflect inferred competence, adherence to norms, and perceived
orientation toward the user’s interests. METI also provides a validated
instrumental basis for measuring these dimensions in a way that can detect
selective shifts, such as competence-related penalties that do not
necessarily generalize to integrity or benevolence.

At the same time, epistemic trust measures targeting a human expert do not
by themselves address how trust is distributed across multiple entities when
an AI system is present. Applied work in advisory and healthcare contexts
demonstrates the value of measuring trust separately for different targets.
Riedl et al. \cite{riedl2024patients} show that participants can provide
meaningful trust evaluations for a human professional, an AI system, and a
hybrid configuration using consistent item structures. While their study is
vignette-based and does not track trust changes through an unfolding
interaction, it provides methodological precedent for entity-specific trust
measurement that can separate evaluations of individuals from evaluations of
a combined system.

This combination of measurement perspectives supports a central feature of
our design. We measure epistemic trustworthiness for the human advisor using
METI, allowing us to test whether competence-related judgments shift in
response to observed performance and correction. We also measure trust for
distinct targets, namely the advisor, the AI assistant, and the advisor-AI
team, enabling us to test whether trust consequences are borne primarily by
the human advisor or are distributed across the human, the AI, and the
combined system. This is particularly important in workflows where AI
oversight is present, because the same correction episode might plausibly be
interpreted as evidence of AI competence, evidence of advisor diligence, or
evidence of advisor failure, depending on how the intervention is initiated
and made visible.

Finally, the workflow-level perspective emphasized in the above literature
suggests that trust measurement should align with the unit of manipulation.
If the independent variable is a complete advising workflow, rather than a
single isolated cue, then the interpretation of trust outcomes should be
grounded in the combined evidence the workflow supplies. This aligns with
treating trust as an interactional judgment shaped by observed outcomes and
procedural cues, and it supports interpreting differences in trust targets
and dimensions as reflections of how participants attribute epistemic
responsibility within the advisory process.




==> Original-Sections/study.tex <==
\subsection{Study Design}
\label{subsec:study-design}

The study was designed to examine how trust judgments form in response to
observed advising outcomes and patterns of AI involvement. Accordingly,
each condition represents a distinct advising workflow that bundles advisor
performance and AI involvement into a single scripted interaction. These
elements were not manipulated as independent experimental factors.
Instead, conditions were constructed as complete advising workflows with
paired sources of variation, reflecting realistic patterns of advising
behavior and AI use as they might occur in practice. This design enables
targeted comparisons between practice-relevant workflows (e.g.,
success vs.\ failure under comparable AI involvement, or different AI
integration strategies under like outcomes) without decomposing the
interaction into factorial main effects.

Participants engaged in a simulated academic advising interaction (Fig.~\ref{fig:workflows}) presented
as a sequence of screenshots and system messages within a web-based
interface~\cite{qualtrics},
(Fig.~\ref{fig:simulation_interface}). They were first presented with a brief description of the study’s
purpose and procedure. Then they were informed that the study involved
interacting with an AI-supported academic advisor and that the
researchers were interested in understanding perceptions of this
interaction in order to inform the effective integration of AI into
everyday contexts. Participants were told that they would complete a course schedule
planning task using the system and informed that the AI system, when
present, acted in an oversight capacity with respect to the advisor. In all conditions, participants were
instructed to assume the role of the student. The participant’s task was to follow
the guidance provided in the interaction
without independently verifying degree requirements or prerequisites.

A between-subjects design was chosen to
avoid carryover and learning effects, particularly given that trust
judgments are known to recalibrate based on prior system performance. Each
participant completed the task once and was randomly assigned to one of five
predefined experimental conditions.


Participants then completed the assigned advising workflow described in
Fig.~\ref{fig:workflows}, proceeding at their own pace through the scripted
interaction. Once the advising interaction was complete, participants were
directed to a post-task questionnaire assessing their perceptions of the
advising experience, including trust-related evaluations of the advisor,
the AI system, and their combination.

The target sample size ($N=77$) was determined a priori through a power
analysis to ensure sufficient sensitivity to detect differences in trust
outcomes across conditions.

\begin{figure*}[t]
  \centering
  \begin{minipage}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/adv_only_succ.jpg}
    \Description{Advisor-only workflow without AI involvement.}
  \end{minipage}\hfill
  \begin{minipage}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/initiated.jpg}
    \Description{Advisor-initiated AI assistance following a detected error.}
  \end{minipage}\hfill
  \begin{minipage}[t]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/automatic.jpg}
    \Description{Automatic AI oversight that continuously monitors and intervenes.}
  \end{minipage}

  \caption{
  Interaction workflows for the advising paradigms examined in this study.
  (Left) \texttt{adv\_only\_succ}: advisor-only workflow without AI involvement.
  (Middle) \texttt{init\_fail}: advisor-initiated AI assistance following a detected error.
  (Right) \texttt{auto\_fail}: automatic AI oversight that continuously monitors and intervenes during the interaction.
  }
  \label{fig:workflows}
\end{figure*}

The five experimental conditions were as follows (illustrative workflows
available in Fig.~\ref{fig:workflows}):

\begin{description}[
  style=unboxed,
  leftmargin=0pt,
  labelsep=0.6em,
  font=\ttfamily\bfseries,
  topsep=4pt,
  partopsep=0pt,
  itemsep=1pt,
  parsep=0pt
]
  \item[init\_succ:] the advisor produces a correct schedule without error,
  with AI present but not making a corrective intervention.
  \item[init\_fail:] the advising workflow contains a scheduling error, with
  correction initiated by the advisor through AI assistance.
  \item[adv\_only\_succ:] the advisor produces a correct schedule without any
  AI involvement.
  \item[auto\_succ:] the advisor produces a correct schedule, with AI
  automatically supervising the interaction.
  \item[auto\_fail:] the advisor produces an incorrect schedule that is
  automatically flagged and corrected by the AI.
\end{description}

Figure~\ref{fig:simulation_interface} illustrates the advising interface
used in the study.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/simulation_interface.png}
\caption{Screenshot of the academic advising simulation interface used in the study. Across conditions, participants interacted with a common advising layout in which guidance was delivered through advisor messages and, when applicable, AI feedback displayed within the advising panel. Differences between conditions were implemented through the availability and behavior of AI intervention mechanisms --- including whether AI feedback was triggered automatically or initiated by the advisor via an on-screen control --- rather than through substantive changes to the overall interface structure or visual design.}
\label{fig:simulation_interface}
\end{figure}



==> Sarath-Sections/Results/analysis.tex <==
\subsection{Overview of Analytical Approach}
%Throughout this section, we distinguish between advisor-targeted trust,
%measured using the Riedl instrument, and global trust, measured using a
%single-item 1-100 scale.

For each measure, we conducted a one-way omnibus analysis of
variance (ANOVA) with condition as the independent variable. Outcomes
included \citet{hendriks2015meti} expertise, integrity, and benevolence composites, the entity-level trust measure adapted from prior work \citet{riedl2024patients}, a general
trust rating assessed on a 1-100 scale, and a behavioral intention measure
assessing participants’ likelihood of reusing the advisor. When an omnibus
test indicated a statistically significant effect, we followed with Tukey’s
HSD for post hoc pairwise comparisons. Effect sizes were estimated using
eta-squared ($\eta^2$) and Cohen's d, respectively. We report test statistics in standard ANOVA form
with exact degrees of freedom, and numerical values are reported alongside
the finalized analyses.

\subsection{Omnibus Tests Across Trust Constructs}
ANOVA analyses were conducted to evaluate omnibus effects of condition across our various measures corresponding to the proposed hypotheses. 

In partial support of H1, no significant effect of condition was observed for the aggregated \citet{hendriks2015meti} composite measure of epistemic trust in the advisor. However, a significant omnibus effect of condition was observed for the \citet{riedl2024patients} advisor-focused trust measure, $F(4,72)=2.64$, $p=.04$, $\eta^2=.13$, indicating that advisor trust judgments varied across workflows on this measure.

Consistent with H2, a significant effect of condition emerged for perceived epistemic expertise of the advisor, $F(4,72)=2.86$, $p=.03$, $\eta^2=.14$. Descriptively, expertise ratings were lowest in the proactive AI failure condition (\procfail), and post-hoc Tukey comparisons showed that the advisor-only success condition (\advonly) was rated significantly higher than \procfail. It is worth noting that the same isn't seen in cases where the advisor correctly identifies a schedule while using an AI assistant. 

No significant omnibus effects were observed for the \citet{hendriks2015meti} dimensions of benevolence or integrity (all $p$s $>.05$), providing no support for H4 or H5. 

In line with H6, the generalized trust rating did not differ significantly across conditions, $F(4,72)=2.447$, $p=.0539$. 

Finally, a significant omnibus effect of condition was observed for participants' reported likelihood of reusing the advisor, $F(4,72)=3.43$, $p=.013$, $\eta^2=.16$. Post-hoc comparisons indicated that reuse intentions were significantly lower only in the proactive-AI failure condition relative to both the advisor-only success and proactive-AI success conditions, providing partial support for H7. 

Across all constructs exhibiting significant omnibus effects, effect sizes were consistently in the medium range ($\eta^2=.13$-.16). No significant omnibus effects were observed for trust measures associated with AI-only or hybrid advisory configurations.

\subsection{Descriptive Statistics}
Table~\ref{tab:descriptives} reports descriptive statistics (mean $\pm$ SD) for trust constructs that exhibited significant omnibus effects: perceived epistemic expertise, aggregated trust, and likelihood of advisor reuse.

Across conditions, perceived expertise ratings were consistently lower in
workflows that contained scheduling errors than in workflows that resulted
in a correct schedule. A similar pattern was observed for aggregated trust
and likelihood of advisor reuse, with error-containing conditions evaluated
less favorably on average than successful advising workflows. 

These descriptive patterns are reported to contextualize the omnibus and post-hoc
tests reported below.


\begin{table}[t]
\centering
\caption{Descriptive statistics (mean $\pm$ SD) for key trust outcomes by condition}
\label{tab:descriptives}
\begin{tabular}{lccc}
\toprule
Condition & METI Expertise & Riedl Trust & Reuse \\
\midrule
\procsucc       & 6.01 $\pm$ 1.11 & 6.00 $\pm$ 1.04 & 6.22 $\pm$ 1.11 \\
\procfail       & 4.99 $\pm$ 1.57 & 4.90 $\pm$ 1.89 & 4.69 $\pm$ 2.12 \\
\advonly  & 6.36 $\pm$ 0.90 & 6.12 $\pm$ 1.35 & 6.36 $\pm$ 1.21 \\
\reactsucc       & 6.01 $\pm$ 0.88 & 6.18 $\pm$ 0.79 & 6.00 $\pm$ 1.12 \\
\reactfail      & 5.58 $\pm$ 1.27 & 5.56 $\pm$ 1.26 & 5.27 $\pm$ 1.62 \\
\bottomrule
\end{tabular}
\end{table}




\subsection{Pairwise Condition Comparisons}
For all Tukey HSD pairwise comparisons, mean differences are computed as
(condition$_2$ $-$ condition$_1$). Thus, negative values indicate higher
ratings in the first-listed condition.

Post-hoc pairwise comparisons were conducted for trust constructs that
exhibited significant omnibus effects. For perceived epistemic expertise,
Tukey HSD tests indicated that advisors in the \advonly\ 
condition were rated as significantly more expert than those in the
\procfail\ condition (mean difference = \text{-1.37}, 95\% CI =
[\text{-2.67}, \text{-0.07}], $p = \text{0.03}$). No other
pairwise comparisons for expertise reached statistical significance. 

For the entity-level trust measures, pairwise comparisons revealed that
participants rated the advisor in the  \procsucc condition as significantly more
trustworthy than the \reactfail condition (mean difference =
\text{-1.28}, 95\% CI = [\text{-2.55}, \text{-0.01}], $p =
\text{0.05}$). 
%Again, this provides credence to H2b, but we don't see any strong evidence for either H2a or H2c.

For the likelihood of advisor reuse, Tukey HSD post-hoc tests indicated that reuse
intentions were significantly higher in the \advonly\ 
condition than in the \reactfail\ condition (mean difference
$= -1.68$, 95\% CI [$-3.31, -0.04$], adjusted $p = 0.04$). Reuse intentions were
also significantly lower in the \procfail\ condition than in the
\procsucc\ condition (mean difference $= 1.53$, 95\% CI
[$0.10, 2.97$], adjusted $p = 0.03$).

==> Sarath-Sections/abstract.tex <==
The increasing integration of AI-powered tools into expert workflows, such as medicine, law, and finance, raises a critical question: how does AI involvement influence a user’s trust in the human expert, the AI system, and the human-AI team? This question is especially important in expert advisory settings where users are epistemically dependent on human-AI systems: they are recipients of guidance produced by an expert using AI support, but often lack the domain knowledge needed to independently verify the recommendation. We investigated these dynamics through a user study ($N=157$) using a simulated course-planning task. Our design varied advisor performance and the structure of AI involvement, including whether AI support was present and, when present, whether it was invoked by the advisor or automatically monitored the interaction. Across all conditions, workflows ultimately produced correct schedules. Results show an asymmetric trust effect: advisor errors significantly reduce trust in the human advisor, but visible AI correction does not produce a corresponding increase in trust toward the AI assistant. Trust judgments remain anchored to the advisor across multiple trust measures, and changing the visible structure of AI involvement does not substantially redistribute trust toward the AI assistant or the human-AI team. These findings suggest a limit of corrective AI as a governance mechanism: making AI oversight visible may improve workflow recoverability, but it does not necessarily redistribute trust or responsibility away from the human-facing expert. In epistemically dependent settings, correctness alone may be insufficient for trustworthy AI integration, as users may continue to assign responsibility to the human expert even when AI assistance visibly shapes the final outcome.

==> Sarath-Sections/hypotheses.tex <==
\section{Hypotheses}
\label{subsec:hypotheses}

Our experiments test four hypotheses motivated by prior work on trust in automation~\cite{lee2004trust, Dzindolet2003Trust, hoff2015trust} and by our directional expectations about how expert missteps and recovery influence trust. Conditions are defined by AI modality (none, proactive, reactive) and advisor performance (errorless, error-present), yielding six conditions: \advonly{}, \advonlyerr{}, \procsucc{}, \procfail{}, \reactsucc{}, and \reactfail{} (see Section~\ref{subsec:study-design}).

In all conditions, the student \text{\color{red}(participant)} is given a course scheduling task {\color{red}(i.e., preparing a course schedule for a new semester)}, specifies desired courses, and receives a valid schedule. In the no-AI condition, the advisor completes the task unaided (Figure~\ref{fig:intro_workflows}(a)). In proactive conditions, the advisor invokes the AI to verify the scheduling choice, and errors, if present, are identified during verification (Figure~\ref{fig:intro_workflows}(b)). In reactive conditions, the AI automatically intervenes and immediately flags errors (Figure~\ref{fig:intro_workflows}(c)). When no error occurs, the interaction proceeds without an error-correction event.

Dependent variables captured four trust-related outcomes: epistemic trustworthiness assessed via the \citet{hendriks2015meti} questionnaire; entity-level trust in the advisor, AI assistant, and human-AI team adapted from \citet{riedl2024patients}; global trust in the advisor on a 100-point scale; and willingness to reuse the advisor on a 7-point Likert scale (``Extremely unlikely'' to ``Extremely likely''). All hypotheses focus on how advisor performance and AI intervention modality influence these evaluations.

Prior work on trust in automation suggests that observed failures prompt trust recalibration~\cite{Dzindolet2003Trust}. Accordingly, we expect advisor performance (error-present vs errorless) to influence trust-related evaluations of the advisor (H1). We further expect that AI intervention modality (none, proactive, reactive) will influence how trust-related evaluations are allocated across the advisor, AI assistant, and advisor-AI team (H2), consistent with frameworks emphasizing how agency and decision authority are distributed in human-automation workflows~\cite{Parasuraman2000TypesLevelsAutomation}. In this framework, differences in who initiates action (e.g., monitoring and verification) reflect different allocations of decision authority, which may influence how observers interpret an advisor’s epistemic responsibility even when task outcomes are identical. \textcolor{blue}{More specifically, visible participation in verification and error detection provides evidence about which entities contribute to the reliability of the final recommendation. When an AI assistant visibly identifies an invalid choice or safeguards the workflow, users may treat that intervention as evidence of the AI assistant’s competence and of the combined advisor-AI team’s capacity to produce dependable guidance. This expectation is consistent with work showing that users distinguish among human, AI, and hybrid trust targets and can evaluate their contributions separately (Riedl, Hogeterp, and Reuter 2024). We therefore expected AI-supported workflows to shift some trust-related credit away from the advisor alone and toward the AI assistant or advisor-AI team. Because reactive AI monitors the interaction independently, whereas proactive AI is invoked at the advisor’s discretion, reactive oversight may provide a stronger cue of independent AI agency and verification authority.} 

\textcolor{blue}{We also expect AI intervention modality to shape how strongly an observed advisor error affects trust in the advisor (H3). Prior work suggests that trust responses depend not only on whether an error occurs, but also on how limitations, feedback, and recovery are communicated within the interaction (Dzindolet et al. 2003; Hoff and Bashir 2015). In an advisor-only workflow, an error may be interpreted primarily as evidence of advisor fallibility. In an AI-supported workflow, however, successful detection and correction may provide a countervailing signal that the broader advisory process contains safeguards capable of recovering from mistakes. The strength of this signal may depend on the intervention structure: advisor-invoked verification may indicate responsible use of a support tool, whereas automatic monitoring may indicate that error detection does not depend on the advisor recognizing the need for assistance. We therefore expect the trust penalty associated with advisor errors to vary across intervention modalities, with AI oversight potentially attenuating the decline relative to an advisor-only workflow. Finally, we expect advisor errors to reduce users’ willingness to reuse the advisor (H4).}



\subsection{Hypotheses List}
\label{hypotheses}

To summarize, the hypotheses we tested are as follows:
\begin{itemize}
    \item H1: Advisor errors will have a significant negative effect on trust-related evaluations of the advisor, including epistemic trustworthiness measured using the \citet{hendriks2015meti} instrument and entity-specific trust adapted from \citet{riedl2024patients}.
    
    \item H2: AI intervention modality (none, proactive, reactive) will significantly affect how trust-related evaluations are distributed across available trust targets, with AI-supported workflows expected to produce higher evaluations of the AI assistant and advisor-AI team when those targets are present.

    \item H3: The trust penalty associated with advisor errors will differ significantly depending on the AI intervention modality.

    \item H4: Participants will be significantly less likely to reuse advisors who made errors than advisors who did not, consistent with prior work linking trust to downstream reliance.
\end{itemize}

As reported below and in Section~\ref{sec:results}, H1 and H4 were supported: advisor performance significantly influenced advisor-directed trust evaluations across multiple measures, including epistemic trustworthiness~\cite{hendriks2015meti}, entity-specific trust~\cite{riedl2024patients}, general trust~\cite{lee2004trust}, and willingness to reuse~\cite{liao2022designing}. H2 and H3 were not supported: AI intervention modality did not produce significant main effects, nor did it significantly moderate the trust penalty associated with advisor errors.

We treat these deviations from the a priori expectations as theoretically informative, suggesting that observed advisor error played a more dominant role than AI involvement strategy in shaping trust and reuse judgments.

==> Sarath-Sections/introduction.tex <==
\section{Introduction}

Across domains such as healthcare, financial advising, legal consultation, and others, people depend on human experts to help them navigate complex decisions~\cite{agrawal2023crosscultural, HanKo2025TrustDynamicsFA, mayer1995integrative, kaye2004roles}. These interactions depend on trust in experts~\cite{hendriks2015meti}: an evaluative judgment that an advisor will help achieve a user’s goals under conditions of uncertainty~\cite{lee2004trust}, which in practice often manifests in reliance behaviors such as reuse~\cite{liao2022designing}. Understanding how trust is shaped within human-AI workflows is therefore critical for interpreting user perceptions and anticipating downstream reliance behavior.

As AI systems increasingly enter expert advisory workflows, users may attribute guidance to the human advisor, the AI system, or the human-AI workflow as a whole. This creates a puzzle for corrective AI: when AI helps identify or resolve an expert error{\color{red}{, which happens when the human expert fails to catch timing or prerequisite issues in the course schedule}}, does it earn trust as a reliable contributor, or does its intervention primarily expose the human expert’s fallibility? Even before a specific intervention occurs, the presence of AI may also shape how users interpret credibility within the advisory process~\cite{nakano2025understanding}. The implications of this shift in advisory contexts remain unclear, and understanding how responsibility and epistemic authority are allocated within such human-AI advisory workflows is central to broader questions of accountability and governance in sociotechnical systems. {\color{red}Throughout this paper, we refer to the human expert as the advisor (or simply the expert), following the academic advising scenario used in our study.} The “user” refers to the recipient of guidance (e.g., a patient {\color{red} or a student}), who does not directly interact with the AI but evaluates the outcomes of a human-AI workflow. As such, the user serves as the trustor, forming judgments about the advisor, the AI system, and their combined behavior. 

% \begin{figure*}[t]
%   \centering
%   \includegraphics[width=\textwidth]{figures/Fig1.png}
%   \caption{Illustrative advising workflows examined in this study, highlighting differences in advisor performance and AI intervention modality.}
%   \label{fig:intro_workflows}
% \end{figure*}


\begin{figure*}[tbp]
  \centering
  \includegraphics[width=0.32\linewidth]{figures/adv_only.jpg}\hfill
  \includegraphics[width=0.32\linewidth]{figures/adv_ai_invoked.jpg}\hfill
  \includegraphics[width=0.32\linewidth]{figures/adv_ai_auto.jpg}
  
  \parbox[t]{0.32\linewidth}{(a)\label{fig:adv_ai_auto} Advisor-only workflow without AI involvement ($C_{adv\_only\_errorless}$ or $C_{adv\_only\_errors}$).}\hfill
  \parbox[t]{0.32\linewidth}{(b)\label{fig:adv_ai_invoked} Advisor-initiated AI correction following an error ($C_{proactive\_errorless}$ or $C_{proactive\_errors}$).}\hfill
  \parbox[t]{0.32\linewidth}{(c)\label{fig:adv_only} Automatic AI oversight and correction ($C_{reactive\_errorless}$ or $C_{reactive\_errors}$).}
  
  \caption{Illustrative advising workflows examined in this study, highlighting differences in advisor performance and AI intervention modality.}
  \label{fig:intro_workflows}
\end{figure*}


Prior work has examined trust in algorithmic systems~\cite{lee2004trust,lee2018understanding} and human experts~\cite{hendriks2015meti}, but less is known about how users distribute trust across human and AI contributors in precision-dependent tasks where both shape the final guidance. This gap is especially important when AI visibly corrects or safeguards expert recommendations, because such interventions may change how users assign credibility and responsibility within the advisory workflow.

From an epistemic perspective, trust in experts can be decomposed into expertise, integrity, and benevolence~\cite{hendriks2015meti}, with advisor performance informing perceived expertise~\cite{tenney2008calibration} and AI oversight potentially shaping integrity- and benevolence-related inferences. This multidimensional approach remains well-justified in trust measurement~\cite{kim2024XAItrust} and is especially relevant for understanding trust in expert AI contexts~\cite{asan2020aiTrustHealthcare}, where AI integration is accelerating~\cite{kaffee2025local,moell2025medical}. In this work, we experimentally manipulate two factors: advisor performance (whether the advisor fails to detect an invalid course selection) and AI oversight modality (advisor-only with no AI involvement, reactive AI oversight that automatically monitors and flags issues, or proactive AI oversight invoked at the human advisor’s discretion). We examine whether and how these factors influence multidimensional trust judgments, entity-specific trust, and downstream behavioral intentions in expert-guided interactions. As we show, these effects are not uniformly distributed across system components, but instead are concentrated in trust judgments directed at the human advisor.

We leveraged an online academic advising simulation as a simplified, representative task to study this phenomenon. Figure~\ref{fig:intro_workflows} provides an overview of the interaction structures considered in our study. Academic advising offers a useful environment for studying these dynamics, since advisors are expected to have expertise and specialized knowledge about courses as well as departmental and university degree requirements~\cite{edutechloft2025_student_advising}. At the same time, while perceived risk is a necessary condition of trust~\cite{mayer1995integrative}, the stakes of advising are moderate enough to limit confounding factors present in higher-risk domains such as medicine or finance, enabling a more controlled examination of trust dynamics. We therefore frame this study, in part, as a mechanism-focused investigation of trust attribution under AI oversight rather than as a direct claim about trust dynamics in all expert domains. Moreover, the scenario naturally supports AI assistants that can run in both a proactive and a reactive mode (Section~\ref{subsec:study-design} provides a full overview of the experiment setup). Each measurement draws on previously validated trust instruments, as described in Section~\ref{subsec:measures}.

Our results show that advisor performance significantly
shapes trust-related evaluations: error-present conditions
were evaluated less favorably across measures of epistemic
trustworthiness, entity-specific trust, general trust, and
likelihood of advisor reuse, even though errors were
ultimately corrected in all conditions, either by the AI system
or the advisor. In contrast, AI intervention modality did not
produce significant effects, suggesting that visible AI
involvement did not substantially redistribute trust away
from the human advisor. Descriptively, performance-related
declines were largest in advisor-only conditions, followed by
proactive AI use, and smallest under reactive AI oversight.
Trust in the AI system remained comparatively stable, with
mixed results for the human-AI team.

Taken together, our results suggest that corrective AI may change how an advisory workflow reaches a valid outcome without changing who users treat as epistemically responsible for that outcome.

\subsection{Contributions}
\label{subsec:contributions}

To summarize, the paper makes three contributions:
\begin{enumerate}
    \item We present an interactive experimental paradigm for studying trust attribution in AI-assisted advisory workflows under controlled variations in advisor performance and AI integration structure.

    \item Using this setup in an academic advising task, we show that observed advisor errors reduced trust in the human advisor, while visible AI correction did not increase trust in the AI assistant despite its role in correcting the error. AI oversight also did not significantly redistribute trust consequences across the advisor, AI assistant, and advisor-AI team, suggesting that epistemic responsibility remained anchored to the human-facing expert. Descriptive patterns suggest that AI involvement may attenuate trust penalties, with heterogeneous responses to advisor mistakes.

    \item We derive design implications for human-AI advisory workflows, emphasizing the importance of advisor competence, real-world constraints on error visibility, the positioning of AI assistance in error detection, and the potential for complementary signals to support adaptive responses to user trust.
\end{enumerate}

==> Sarath-Sections/study.tex <==
\subsection{Study Design}
\label{subsec:study-design}

The study examines how trust judgments form in response to realistic advising sequences and AI involvement. Each participant received a distinct, randomly-assigned workflow varying along two factors: advisor performance and AI intervention modality, allowing us to assess their effects and interaction.

Participants engaged in a simulated academic advising interaction (Fig.~\ref{fig:workflows}) presented as a sequence of screenshots and system messages within a web-based interface~\cite{qualtrics} (Appendix~\ref{app:sim-walkthrough} Figs.~\ref{fig:appendix-sim-seq}, ~\ref{fig:appendix-sim-seq-part2}). They were informed that they would complete a course scheduling task (with or without AI) and that the study examined perceptions of this interaction. The AI, when present, operated in an oversight tool. When errors occurred, they were observable: with AI, they were surfaced through messages and visual {\color{red}text} feedback indicating invalid course selections; without AI, the advisor identified them by cross-referencing a rule book and addressed them in the chat. In all conditions, participants assumed the role of the student and were instructed to follow the guidance. They were never provided means to verify their choices independently. 

A between-subjects design was used to avoid carryover and learning effects, as trust judgments recalibrate based on prior performance~\cite{lee2004trust}. Each participant completed the task once. \textcolor{blue}{Participants completed the assigned advising workflow at their own pace, then completed a post-task questionnaire assessing trust-related evaluations of the advisor. Participants in the AI-supported conditions additionally evaluated the AI assistant and the advisor-AI team.}

\sout{The target sample size ($N=157$) was determined a priori via power analysis to ensure sensitivity to differences in trust outcomes across conditions.} 

\textcolor{blue}{%
An a priori power analysis was conducted in G*Power 3.1.9.7
for the advisor performance $\times$ AI intervention modality interaction.
For the $3 \times 2$ factorial analyses of advisor-directed outcomes,
assuming a medium interaction effect ($f=.25$), $\alpha=.05$, and power
of $.80$, the analysis indicated a required total sample size of $N=158$
across six conditions. The final analytic sample of $N=157$ provided
approximately 79.9\% power under these assumptions. For the $2 \times 2$ factorial analyses restricted to the AI-supported
conditions, the same assumptions indicated a required sample size of
$N=128$ across four conditions. The available AI-supported subsample was
$N=109$, which provided approximately 73.4\% power to detect an interaction
of $f=.25$.
}

The experimental interactions were as follows (illustrative workflows available in Fig.~\ref{fig:workflows}):



\begin{description}
  \item[\advonly{}:] Advisor-only, errorless condition. The student selects courses that satisfy the scheduling requirements, and the advising workflow proceeds without AI involvement.

  \item[\advonlyerr{}:] Advisor-only, error-present condition. The student selects an invalid course, which the advisor detects only after checking the rule book and corrects without AI involvement.

  \item[\procsucc{}:] Advisor-invoked AI, errorless condition. The student selects courses that satisfy the scheduling requirements within a workflow where AI support is available through advisor invocation.

  \item[\procfail{}:] Advisor-invoked AI, error-present condition. The student selects an invalid course that the advisor does not initially detect; advisor-invoked AI assistance identifies the error so it can be corrected before the final schedule is produced.

  \item[\reactsucc{}:] Automatic AI oversight, errorless condition. The student selects courses that satisfy the scheduling requirements within a workflow involving automatic AI oversight.

  \item[\reactfail{}:] Automatic AI oversight, error-present condition. The student selects an invalid course that the advisor does not initially detect; automatic AI oversight flags the error so it can be corrected before the final schedule is produced.
\end{description}

\roya{I think adding this is redundant(it's already being said in the hypos) but just because it was in the comments I put it here for now:}

{\color{red}So, depending on the condition, errors can be caught in three ways. In \advonlyerr, they are caught by the advisor. In \procfail, they are caught through advisor-invoked AI verification. In \reactfail, they are caught through automatic AI monitoring.}

==> commands.tex <==
\newcommand{\reactsucc}{\ensuremath{C_{reactive\_errorless}}}
\newcommand{\reactfail}{\ensuremath{C_{reactive\_errors}}}
\newcommand{\advonly}{\ensuremath{C_{adv\_only\_errorless}}}
\newcommand{\procsucc}{\ensuremath{C_{proactive\_errorless}}}
\newcommand{\procfail}{\ensuremath{C_{proactive\_errors}}}
\newcommand{\advonlyerr}{\ensuremath{C_{adv\_only\_errors}}}


\newcommand{\showcomments}{1}
\newcommand{\roya}[1]{\ifnum\showcomments=1 \textcolor{brown}{[Roya: #1]}\fi}

